VLA-Trace: Diagnosing Vision-Language-Action Models through Representation and Behavior Tracing

Understanding how Vision-Language-Action (VLA) models transform multimodal knowledge into embodied control remains an open challenge. We present VLA-Trace, a progressive diagnostic framework that analyzes VLA models through a unified evidence chain from representation dynamics to causal control attribution and behavioral manifestation. It specifically combines cross-modal and checkpoint-drift centered kernel alignment (CKA) to trace representation evolution, attention knockout interventions to identify modality-specific control pathways, and rollout-level behavioral probes to examine grounding, shortcut dependence, and semantic following. Experiments on $\pi_{0.5}$ and OpenVLA reveal three key findings. First, the two models exhibit distinct modality-specific adaptation dynamics during VLA finetuning. Second, they rely on different multimodal routing strategies and layer-wise dependencies during action decoding. Third, although VLA policies excel at visually grounded trajectory generation, they remain limited in fine-grained semantic following. These findings highlight future directions for representation-preserving adaptation, causal VLA circuits, and compositional semantic control.

==> sections/analysis_framework.tex <==
\section{Representation Analysis Framework}
\subsection{Overview}

We systematically investigate latent representations in VLA models across three developmental stages: (i) a pretrained vision-language model (VLM), which encodes general-purpose semantic and perceptual knowledge; (ii) a pretrained VLA model, adapted from the VLM for action generation using large-scale embodied data; and (iii) a finetuned VLA model, further optimized for downstream robot tasks. This staged formulation provides a principled framework for analyzing how semantic priors acquired during pretraining are preserved, adapted, or distorted as the model transitions from perception and language understanding to embodied control.

Building on this perspective, our analysis proceeds along three key dimensions: (1) stage-wise representation dynamics, (2) visual-language control over action generation, and (3) behavioral manifestations of the identified control pathways. These dimensions form a progressive evidence chain. First, representation analysis identifies where VLA adaptation alters the pretrained semantic space. Second, intervention analysis tests whether the resulting pathways are functionally used for action generation. Finally, behavioral perturbations reveal how these internal pathways affect embodied execution, manifesting as concrete visual shortcuts, local affordance dependencies, or semantic instruction-following failures.

We introduce the concept of \textit{language semantic authority} to evaluate whether language acts as a compositional guide for action rather than a static conditioning scaffold. Operationally, language exhibits semantic authority when semantic instruction tokens (or the representations they induce during prefill) are causally necessary for action generation, and when controlled edits to instruction semantics successfully redirect the policy toward the edited target. A model may attend to text, preserve textual geometry, or require prompt tokens, yet still lack semantic authority if the text functions merely as a template, cache initializer, or rigid conditioning signal.

\subsection{Model and Evaluation Scope}

The VLA-Trace protocol is applicable across multiple VLA architectures and simulation environments, including streaming policies, autoregressive policies, and regression-style action decoders. In this paper, we focus our primary analysis on $\pifive$ and OpenVLA, as they present contrasting inference structures that are highly diagnostic for language and vision utilization. $\pifive$ employs a PaliGemma-based VLM with an action expert and flow-matching action generation. Its transformer input consists of multi-view images, a BOS token, the task instruction, and a newline token, allowing bidirectional visual-language interaction during context formation. Conversely, OpenVLA utilizes an autoregressive Llama-based architecture where image patches are followed by a prompt template (e.g., \textit{``In: What action should the robot take to \{instruction\}? Out:''}). This autoregressive structure introduces structural tokens and attention sinks that must be carefully isolated from semantic instruction tokens during intervention.

Our primary experiments utilize COCO as an open-domain image-text reference and the LIBERO suites as robot-domain evaluation environments, incorporating Simpler patch-masking results where available. While our broader implementation matrix extends to Calvin, LIBERO-Plus/Pro, RoboTwin, X-VLA, and OpenVLA-OFT, we focus on the $\pifive$/OpenVLA and COCO/LIBERO settings to present a complete and coherent evidence chain.

\subsection{Stage-wise Representation Dynamics (RQ1)}

The first stage analyzes the transformation of latent representations to determine whether robot-domain training improves general vision-language alignment or reshapes pretrained semantic spaces. We compare $\pifive$ across C0/C1/C2 checkpoints and OpenVLA across raw and finetuned checkpoints.

\textbf{\textit{(1) Cross-modal CKA.}} To quantify vision-language alignment, we compute linear Centered Kernel Alignment (CKA) between pooled visual and textual representations at each layer. For the CKA inputs, LIBERO instructions are converted to the text template \texttt{A photo of a robot \textless instruction\textgreater}, while COCO captions use \texttt{A photo of \textless caption\textgreater}. This keeps the CKA probe in an image-description format for both robot-domain and open-domain data, while preserving the semantic content of the original instruction or caption. The metric evaluates whether image and language tokens share similar sample-level geometry, enabling us to distinguish between distributed cross-modal alignment and terminal-layer spike alignment.

\textbf{\textit{(2) Checkpoint Drift CKA.}} To assess representation stability, we compute CKA between the same layer across different training stages for visual, textual, and joint pooled states. A high drift CKA indicates subspace preservation, whereas a low value signifies substantial rewriting. This metric reveals whether robot adaptation degrades or restructures the language-related subspace. We treat CKA as a geometric diagnostic rather than a behavioral metric; it compares representations without requiring neuron-wise alignment, though it does not guarantee identical decision boundaries.

\textbf{\textit{(3) Modality-level Attention Statistics.}} We measure how action queries allocate attention to image, text, action, and structural tokens. This provides an intermediate bridge between representation geometry and intervention analysis, while also exposing special-token sinks that can artificially inflate apparent language grounding.

Formally, let $A^{(l,h)} \in \mathbb{R}^{N_q \times N_k}$ denote the attention matrix at layer $l$ and head $h$, and let $Q_A$ be the set of action-query tokens. For any token subset $S$ such as image patches, instruction tokens, BOS/newline tokens, prompt-template tokens, or action tokens, we summarize action-to-subset routing as
\begin{equation}
\mathrm{Mass}^{(l)}(S)=
\frac{1}{|H_l|\,|Q_A|}
\sum_{h\in H_l}\sum_{i\in Q_A}\sum_{j\in S} A^{(l,h)}_{ij}.
\label{eq:modality_mass}
\end{equation}
This statistic is descriptive rather than causal: high mass indicates that action tokens route information through a subset, but does not by itself show that the subset is necessary for task success. We therefore use it only as a bridge between CKA geometry and the causal knockout tests below.

\textbf{\textit{(4) Attention IoU for Visual Grounding.}} To quantify attention localization, we compute the overlap between high-attention visual patches and simulator-derived object or robot masks. This Attention IoU probe tests whether action attention is spatially aligned with task-relevant affordances rather than merely tracking visual saliency.

\subsection{Visual-Language Control over Action (RQ2)}

The second stage localizes the visual-language control bottleneck by probing how latent representations causally influence action generation. The objective is to distinguish representational availability from functional necessity. Following the staged design in our implementation protocol, we decompose inference into representation formation and action decoding, and perform targeted attention interventions at each stage. This allows us to determine whether a modality contributes by shaping the initial multimodal context, by directly conditioning the action tokens during decoding, or by both mechanisms.

\textbf{\textit{(1)~Prefill (Cross-modal Interaction).}}
The prefill stage encodes all input modalities (vision and language) to construct the initial internal representations. To isolate the role of cross-modal interaction, we intervene by blocking attention between vision and language tokens (V–L attention), thereby enforcing independent modality processing. This allows us to assess how cross-modal integration during representation formation influences downstream action generation. In Pi0.5 with bi-directional attention, for example, given concatenated vision and language tokens $X = [X^L;X^V]$, we compute self-attention as:
\begin{equation}
\mathrm{Attn}(Q, K, V) = \mathrm{softmax}\left(\frac{QK^\top}{\sqrt{d}} + M \right)V.
\end{equation}
where $M^l$ is a textual block mask at layer $l$ to prevent cross-modal attention
% \begin{equation}
% M^{l} =
% \begin{bmatrix}
% \mathbf{LL} & -\infty \\
% -\infty & -\infty
% \end{bmatrix},
% \end{equation}
\begin{equation}
M^{l} =
\begin{bmatrix}
\mathbf{LL} & -\infty & \mathbf{LA} \\
-\infty & \mathbf{VV} & \mathbf{VA} \\
\mathbf{AL} & \mathbf{AV} & \mathbf{AA}
\end{bmatrix},
\end{equation}
ensuring that vision and language tokens are processed independently.

\textbf{\textit{(2)~Generation (Modality Dependency).}}
In the generation stage, actions are produced autoregressively. We perform a modality knockout by blocking attention from action tokens to vision or language tokens, preventing the model from conditioning on multimodal context during decoding. This intervention isolates the extent to which action generation depends on vision-language information at inference time. The textual mask at layer $l$ can be described as:
\begin{equation}
M^{l} =
\begin{bmatrix}
\mathbf{LL} & \mathbf{LV} & -\infty \\
\mathbf{-} & \mathbf{VV} & \mathbf{VA} \\
\mathbf{-} & \mathbf{-} & \mathbf{AA}
\end{bmatrix},
\end{equation}

This design allows us to disentangle two fundamentally different roles of multimodal information in VLA models: 
(i) cross-modal interaction during representation formation in the encoding stage, and 
(ii) modality dependency during action generation in the decoding stage. 
By intervening at these two stages, we can distinguish whether performance gains arise from better multimodal understanding or more effective utilization of modality-specific information during generation. Three attention configurations are considered: \textbf{i.} Baseline, where all modalities are provided; \textbf{ii.} No Image, where visual attention is removed; \textbf{iii.} No Text, where language attention is excluded.

Model performance is evaluated using success rate ($\%$). For each task, 20 trials are conducted across 10 tasks on LIBERO-10, resulting in a total of 200 evaluation episodes.

\textbf{\textit{(3) Attention Pattern Analysis.}} Following knockout, we visualize how action tokens allocate attention to image regions, instruction tokens, and camera views during closed-loop rollouts. This clarifies how necessary pathways are routed within the transformer and whether they align with task stages or collapse onto visual/formatting sinks.

\subsection{Behavioral Manifestation of Control Pathways (RQ3)}

The final stage tests whether the internal pathways identified by CKA and knockout correspond to observable execution shortcuts or semantic failures, thereby validating the practical relevance of our diagnostic toolchain.

\textbf{\textit{(1) Visual Patch Masking.}} We selectively mask target objects, gripper regions, robot bodies, and backgrounds using background-color replacement, black masking, and mosaic masking. Because these methods remove different amounts of information (e.g., background replacement removes appearance and boundary cues, while mosaic preserves partial spatial structure), comparing success rates reveals whether the policy relies on fine-grained object appearance, coarse shape, or local gripper-object geometry.

\textbf{\textit{(2) Attention IoU and Visualization.}} We compute thresholded Top-10 patch IoU, continuous attention mass, and peak-hit rates to determine whether the most attended visual patches overlap with task-relevant masks. These metrics verify whether action attention dynamically tracks active subtask objects or remains statically fixed on generic visual features.

\textbf{\textit{(3) Input Editing.}} We modify object positions or replace object mentions in the instruction while preserving the overall task template. If a model maintains language as a compositional guide, such edits should redirect its actions accordingly. Failure to follow edited targets indicates semantic forgetting or a rigid coupling between the original prompt and the scene layout.



==> sections/cka_knockout.tex <==
\subsection{Stage-wise Representation Dynamics}
\label{subsec:cka_representation}

This section addresses \textit{\textbf{RQ1:} How do latent representations dynamically evolve across the deeper layers of VLA?} We first analyze whether vision-language alignment is strengthened, preserved, or reshaped when a pretrained multimodal model is adapted into a robot policy. To this end, we use linear centered kernel alignment (CKA), which compares sample-level representation geometry without requiring neuron-wise correspondence across modalities or checkpoints. Given two representation matrices $X \in \mathbb{R}^{N \times d_x}$ and $Y \in \mathbb{R}^{N \times d_y}$, linear CKA is computed as:
\begin{equation}
\mathrm{CKA}(X,Y)=
\frac{\lVert X^\top Y \rVert_F^2}
{\lVert X^\top X \rVert_F \lVert Y^\top Y \rVert_F}.
\end{equation}
We consider two complementary measurements. \textbf{\textit{(1) Cross-modal CKA.}} For each layer $l$, we compute CKA between the pooled visual representation $H_l^V$ and pooled textual representation $H_l^T$, which measures whether visual and textual tokens share similar sample geometry. The textual side is constructed with dataset-specific description templates: LIBERO uses \texttt{A photo of a robot \textless instruction\textgreater}, and COCO uses \texttt{A photo of \textless caption\textgreater}. \textbf{\textit{(2) Checkpoint-drift CKA.}} For each visual, textual, and joint representation view, we compute CKA between the same layer across checkpoints, which reflects how much the corresponding subspace is preserved or rewritten during VLA pretraining and robot-domain finetuning. Cross-modal CKA characterizes the layer-wise shape of alignment, while drift CKA indicates whether this alignment is obtained by preserving pretrained semantic geometry or by replacing it with robot-domain representations.

\begin{figure*}[ht!]
    \centering
    \includegraphics[width=\textwidth]{figs/cross_modal_cka_grid.png}
    \caption{Layer-wise cross-modal CKA across models, datasets, and training stages. The grid shows both the magnitude and depth profile of image--text alignment. $\pifive$ develops a broad early-to-middle alignment band after VLA pretraining, whereas OpenVLA keeps most intermediate layers weakly aligned and concentrates robot-domain alignment at the terminal layer. The COCO column serves as an open-domain contrast to the robot-domain LIBERO suites.}
    \label{fig:cross_modal_cka_grid}
\end{figure*}

\begin{table*}[ht!]
\centering
\scriptsize
\begin{tabular}{llccccc}
\toprule
Model & Stage & COCO & LIBERO-10 & LIBERO-goal & LIBERO-spatial & LIBERO-object \\
\midrule
\multirow{3}{*}{$\pifive$} 
& C0 & 0.249 / \textbf{0.375}@L13 & 0.684 / \textbf{0.861}@L12 & 0.301 / \textbf{0.507}@L12 & 0.490 / \textbf{0.687}@L14 & 0.672 / \textbf{0.773}@L14 \\
& C1 & 0.351 / \textbf{0.659}@L1 & 0.707 / \textbf{0.924}@L2 & 0.486 / \textbf{0.872}@L15 & 0.513 / \textbf{0.745}@L15 & 0.548 / \textbf{0.814}@L2 \\
& C2 & 0.388 / \textbf{0.664}@L2 & 0.535 / \textbf{0.758}@L2 & 0.486 / \textbf{0.789}@L2 & 0.576 / \textbf{0.833}@L18 & 0.693 / \textbf{0.946}@L1 \\
\midrule
\multirow{2}{*}{OpenVLA} 
& C1 & 0.044 / \textbf{0.501}@L32 & 0.486 / \textbf{0.890}@L32 & 0.042 / \textbf{0.478}@L32 & 0.215 / \textbf{0.727}@L32 & 0.194 / \textbf{0.650}@L32 \\
& C2 & 0.038 / \textbf{0.493}@L1 & 0.463 / \textbf{0.922}@L32 & 0.043 / \textbf{0.787}@L32 & 0.169 / \textbf{0.909}@L32 & 0.116 / \textbf{0.873}@L32 \\
\bottomrule
\end{tabular}
\caption{Layer-mean / peak cross-modal CKA across training stages. Peak layer is shown after @. The layer mean describes the overall thickness of alignment across depth, while the peak value and its layer identify where the strongest linear image--text coupling occurs.}
\label{tab:cka_summary}
\end{table*}

\begin{figure*}[ht!]
    \centering
    \includegraphics[width=0.88\textwidth]{figs/peak_cka_bars.png}
    \caption{Peak cross-modal CKA comparison across checkpoints and evaluation distributions. The bar chart makes the stage-wise specialization visible: $\pifive$ gains broad alignment from C0 to C1, but C1$\rightarrow$C2 finetuning decreases the peak on LIBERO-10 and LIBERO-goal while increasing it on LIBERO-spatial and LIBERO-object. OpenVLA strengthens terminal-layer peaks on robot-domain LIBERO suites but not on open-domain COCO.}
    \label{fig:peak_cka_bars}
\end{figure*}

\subsubsection{Vision-Language Alignment}
As illustrated in Figure~\ref{fig:cross_modal_cka_grid}, Figure~\ref{fig:peak_cka_bars}, and Table~\ref{tab:cka_summary}, CKA reveals that VLA adaptation is not a uniform process of increasing image--text alignment. We interpret these values as relative trends and layer-wise profiles rather than absolute grounding scores, because CKA can be influenced by representation anisotropy, pooling, and dataset composition. Under this interpretation, $\pifive$ shows its largest shift before the final robot-domain finetuning stage. Moving from the original PaliGemma VLM checkpoint (C0) to the VLA-pretrained checkpoint (C1), the peak CKA rises on every evaluated distribution: COCO increases from 0.375 at L13 to 0.659 at L1, LIBERO-10 from 0.861 at L12 to 0.924 at L2, LIBERO-goal from 0.507 at L12 to 0.872 at L15, LIBERO-spatial from 0.687 at L14 to 0.745 at L15, and LIBERO-object from 0.773 at L14 to 0.814 at L2. The layer-mean values also become higher on COCO, LIBERO-10, LIBERO-goal, and LIBERO-spatial. This pattern indicates that \ul{the broad cross-modal geometry used by $\pifive$ is largely built during VLA pretraining rather than being created from scratch by the final robot finetuning stage.}

The subsequent C1$\rightarrow$C2 transition is more diagnostic because it separates general VLA pretraining from task-specialized robot adaptation. For $\pifive$, finetuning does not monotonically strengthen alignment. COCO, LIBERO-spatial, and LIBERO-object increase to peak CKA values of 0.664, 0.833, and 0.946, respectively, whereas LIBERO-10 and LIBERO-goal decrease to 0.758 and 0.789. Because the same $\pifive$ C2 checkpoint is evaluated across these suites, the suite-level difference should not be interpreted as separate weight changes. Instead, it shows that the post-finetuning representation exposes different alignment geometry depending on the semantic breadth of the evaluation distribution. Narrower object- or spatial-centric tasks can produce very high local image--text correspondence, while broader multi-task or goal-level distributions expose weaker and less stable correspondence. In this sense, CKA suggests a specialization trade-off: robot finetuning can sharpen alignment for constrained control patterns while reducing the apparent breadth of generic semantic alignment.

OpenVLA follows a qualitatively different route. Its cross-modal CKA stays low through most layers and rises sharply near the final layer, producing a terminal spike rather than the thicker early-to-middle alignment band observed in $\pifive$. After LIBERO finetuning, the final-layer peak increases on every robot-domain suite: LIBERO-10 improves from 0.890 to 0.922, LIBERO-goal from 0.478 to 0.787, LIBERO-spatial from 0.727 to 0.909, and LIBERO-object from 0.650 to 0.873. The same trend does not hold on COCO, where the peak slightly decreases from 0.501 to 0.493 and moves from L32 to L1. This contrast is important for the paper's argument: \ul{OpenVLA finetuning appears to strengthen a robot-domain terminal fusion mechanism, but that mechanism does not transfer cleanly to open-domain image--text inputs.} The result is consistent with a late-fusion autoregressive interface in which intermediate layers preserve relatively separated visual and textual geometry, and the model performs a sharp alignment operation close to action decoding.

The architecture-level difference is therefore not only a difference in absolute CKA score, but a difference in where the model pays the cost of multimodal fusion. $\pifive$, with bidirectional multimodal attention, can establish cross-modal coupling early and maintain a distributed alignment band across depth. OpenVLA, built around a unidirectional language-model backbone, keeps most of the backbone weakly aligned and concentrates image--text interaction at the end. This distinction explains why the same high-level term, ``vision-language alignment,'' should not be treated as a single scalar property in VLA models. A high final-layer peak may reflect a narrow task-specific fusion interface, whereas a higher layer mean indicates broader representational coupling across depth. VLA-Trace therefore reports both layer means and peak layers, because their combination reveals whether adaptation produces a broad semantic geometry or a narrow terminal control interface.

\subsubsection{Checkpoint Drift and Adaptation Pressure}
We further analyze checkpoint-drift CKA to identify which subspaces are preserved and which are rewritten during robot adaptation. As shown in Figure~\ref{fig:pi05_drift}, $\pifive$ exhibits substantially stronger drift in textual representations than in visual representations. From C0 to C2, text drift CKA is 0.337 on LIBERO-10, 0.151 on LIBERO-goal, 0.145 on LIBERO-spatial, and 0.144 on LIBERO-object, while the corresponding vision drift values remain higher at 0.487, 0.223, 0.233, and 0.227. Thus, the textual subspace is not simply preserved as an unchanged instruction encoder. It is heavily reshaped during the construction of an embodied policy, suggesting that language representations may be converted from general semantic descriptions into task-conditioned control features.

OpenVLA displays the opposite pressure allocation. As shown in Figure~\ref{fig:openvla_drift}, textual drift remains extremely high after finetuning, with text CKA of 0.921 on COCO, 0.989 on LIBERO-10, 0.983 on LIBERO-goal, 0.962 on LIBERO-spatial, and 0.979 on LIBERO-object. The main representational changes instead occur in the visual and joint views; for example, joint drift falls to 0.438 on LIBERO-goal, 0.604 on LIBERO-spatial, and 0.537 on LIBERO-object. This pattern suggests that OpenVLA adapts to robot control while leaving the language backbone comparatively rigid, pushing much of the adaptation burden into visual and fusion representations. This is not necessarily a weakness by itself: preserving language geometry can protect linguistic priors. However, it also raises a central question for the next stage of VLA-Trace: if the language space is preserved, is it actually used as a compositional semantic controller, or does the policy rely on prompt-format and visual-fusion shortcuts?

Taken together, cross-modal CKA and drift CKA expose two adaptation regimes. $\pifive$ builds a distributed alignment basis during VLA pretraining, but final robot adaptation rewrites textual and joint spaces and yields suite-dependent alignment specialization. OpenVLA preserves textual geometry but concentrates robot-domain alignment in a terminal fusion layer and shows an open-domain COCO mismatch after finetuning. These representation findings motivate the causal tests in Section~\ref{subsec:attention_knockout}: CKA can identify where representations align or drift, but only attention knockout can test whether these preserved or rewritten pathways are necessary for action generation.

\begin{figure*}[ht!]
    \centering
    \begin{subfigure}[t]{0.49\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figs/pi05_drift_by_suite.png}
        \caption{$\pifive$ drift CKA relative to C0.}
        \label{fig:pi05_drift}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.49\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figs/openvla_drift_by_suite.png}
        \caption{OpenVLA drift CKA relative to C1.}
        \label{fig:openvla_drift}
    \end{subfigure}
    \caption{Checkpoint drift CKA over visual, textual, and joint pooled representations. Lower values indicate stronger representation rewriting after VLA adaptation.}
    \label{fig:drift_cka}
\end{figure*}

\begin{table}[h!]
\begin{tcolorbox}[
    colback=blue!5!white,
    colframe=black,
    width=\linewidth,
    boxrule=0.5pt,
    sharp corners,
    fonttitle=\bfseries,
    coltitle=black,
    before skip=5pt,
    after skip=5pt,
    boxsep=0pt,
    left=5pt, right=5pt, top=5pt, bottom=5pt
]
\noindent \textbf{\textcolor{black}{Summary.}} \small

CKA analysis shows that VLA adaptation is not a uniform improvement of general vision-language grounding. $\pifive$ first builds a broad alignment basis during VLA pretraining, then final robot finetuning produces suite-dependent specialization and substantial text/joint-space rewriting. OpenVLA follows the opposite route: textual geometry remains highly preserved, but robot-domain alignment concentrates in a terminal fusion layer and does not transfer cleanly to open-domain COCO. These patterns motivate the next step of VLA-Trace: testing whether the preserved or rewritten pathways identified by CKA are actually necessary for action generation.
\end{tcolorbox}
\end{table}

\subsection{Visual-Language Control over Action}
\label{subsec:attention_knockout}

This section addresses \textit{\textbf{RQ2:} What signals actually control action generation in VLA models?} In this experiment, we investigate modality contributions in VLA models through an attention-based knockout design. CKA reveals how representations change, but it does not establish whether a representation is functionally used in control; attention knockout therefore serves as the causal counterpart to the representation analysis above. Experiments are conducted on LIBERO-10 and the 0410 LIBERO-goal/object/spatial suites using two representative VLA models, $\pifive$ and OpenVLA. We decompose inference into two stages and perform targeted interventions at each stage. In \textbf{\textit{Prefill (Cross-modal Interaction)}}, the model encodes the visual observation and language instruction into internal context representations; blocking image or vision-language attention tests whether cross-modal interaction is necessary during representation formation. In \textbf{\textit{Generation (Modality Dependency)}}, action tokens are produced; blocking action-token attention to image, text, or structural prompt tokens tests which signals are required during online action decoding. This design disentangles two roles of multimodal information: cross-modal integration before action decoding and modality-specific dependency during action generation. We evaluate success rate ($\%$) over 200 episodes and report both all-layer interventions and layer-wise scans. Table~\ref{tab:knockout_summary} includes LIBERO-10 together with the 0410 suites, while Table~\ref{tab:layerwise_knockout_summary} summarizes the localized layer-wise effects.

\begin{figure*}[ht!]
    \centering
    \begin{subfigure}[t]{0.49\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figs/all_layers_knockout_heatmap.png}
        \caption{All-layer knockout delta.}
        \label{fig:all_layers_knockout}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.49\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figs/layerwise_knockout_heatmap.png}
        \caption{Worst layer-wise drop.}
        \label{fig:layerwise_knockout}
    \end{subfigure}
    \caption{Attention knockout results across models and LIBERO suites. All-layer interventions reveal global modality dependency, while layer-wise interventions localize the most vulnerable control layers.}
    \label{fig:knockout_heatmaps}
\end{figure*}

\begin{table*}[ht!]
\centering
\scriptsize
\setlength{\tabcolsep}{3.5pt}
\begin{tabular}{llllcc}
\toprule
Model & Dataset & Protocol & Intervention & Episodes & SR \\
\midrule
\multirow{38}{*}{$\pifive$}
& LIBERO-10 & baseline & Baseline & 200 & 91.20 \\
& LIBERO-10 & phase & Generation no image & 200 & 86.20 \\
& LIBERO-10 & phase & Generation no text & 200 & 1.40 \\
& LIBERO-10 & phase & Prefill no V--L & 200 & 82.80 \\
& LIBERO-10 & phase & Prefill no image & 200 & 81.20 \\
& LIBERO-10 & phase & Prefill no text & 200 & 80.60 \\
& LIBERO-10 & global & Global no image & 200 & 47.80 \\
& LIBERO-10 & global & Global no text & 200 & 0.40 \\
& LIBERO-10 & global & Global no V--L & 200 & 0.00 \\
& LIBERO-10 & all-layer combo & Prefill no V--L + generation no image & 200 & 0.00 \\
& LIBERO-10 & all-layer combo & Prefill no V--L + generation no text & 200 & 73.50 \\
\cmidrule(lr){2-6}
& LIBERO-goal & all-layer & Baseline & 200 & 97.00 \\
& LIBERO-goal & all-layer & Generation drop BOS+newline & 200 & 97.50 \\
& LIBERO-goal & all-layer & Generation drop instruction & 200 & 97.00 \\
& LIBERO-goal & all-layer & Generation keep BOS+newline only & 200 & 1.50 \\
& LIBERO-goal & all-layer & Generation no image & 200 & 4.00 \\
& LIBERO-goal & all-layer & Generation no text & 200 & 96.50 \\
& LIBERO-goal & all-layer & Prefill no V--L & 200 & 11.50 \\
& LIBERO-goal & all-layer & Prefill no V--L + generation no image & 200 & 0.00 \\
& LIBERO-goal & all-layer & Prefill no V--L + generation no text & 200 & 11.75 \\
\cmidrule(lr){2-6}
& LIBERO-object & all-layer & Baseline & 200 & 98.33 \\
& LIBERO-object & all-layer & Generation drop BOS+newline & 200 & 99.50 \\
& LIBERO-object & all-layer & Generation drop instruction & 200 & 99.50 \\
& LIBERO-object & all-layer & Generation keep BOS+newline only & 200 & 0.00 \\
& LIBERO-object & all-layer & Generation no image & 200 & 0.00 \\
& LIBERO-object & all-layer & Generation no text & 200 & 98.00 \\
& LIBERO-object & all-layer & Prefill no V--L & 200 & 71.50 \\
& LIBERO-object & all-layer & Prefill no V--L + generation no image & 200 & 0.00 \\
& LIBERO-object & all-layer & Prefill no V--L + generation no text & 200 & 46.00 \\
\cmidrule(lr){2-6}
& LIBERO-spatial & all-layer & Baseline & 200 & 99.00 \\
& LIBERO-spatial & all-layer & Generation drop BOS+newline & 200 & 99.00 \\
& LIBERO-spatial & all-layer & Generation drop instruction & 200 & 100.00 \\
& LIBERO-spatial & all-layer & Generation keep BOS+newline only & 200 & 0.00 \\
& LIBERO-spatial & all-layer & Generation no image & 200 & 0.00 \\
& LIBERO-spatial & all-layer & Generation no text & 200 & 99.00 \\
& LIBERO-spatial & all-layer & Prefill no V--L & 200 & 76.25 \\
& LIBERO-spatial & all-layer & Prefill no V--L + generation no image & 200 & 0.00 \\
& LIBERO-spatial & all-layer & Prefill no V--L + generation no text & 200 & 70.67 \\
\midrule
\multirow{32}{*}{OpenVLA}
& LIBERO-10 & baseline & Baseline & 200 & 56.80 \\
& LIBERO-10 & phase & Generation no image & 200 & 1.00 \\
& LIBERO-10 & phase & Generation no text & 200 & 0.00 \\
& LIBERO-10 & phase & Prefill no image & 200 & 0.00 \\
& LIBERO-10 & phase & Prefill no text & 200 & 47.40 \\
& LIBERO-10 & global & Global no image & 200 & 0.00 \\
& LIBERO-10 & global & Global no text & 200 & 0.00 \\
& LIBERO-10 & global & Global no V--L & 200 & 0.00 \\
\cmidrule(lr){2-6}
& LIBERO-goal & all-layer & Baseline & 200 & 77.25 \\
& LIBERO-goal & all-layer & Generation drop newline & 200 & 75.50 \\
& LIBERO-goal & all-layer & Generation drop prompt, keep newline & 200 & 0.00 \\
& LIBERO-goal & all-layer & Generation no image & 200 & 16.00 \\
& LIBERO-goal & all-layer & Generation no text & 200 & 0.00 \\
& LIBERO-goal & all-layer & Prefill no image & 200 & 0.00 \\
& LIBERO-goal & all-layer & Prefill no image + generation no image & 200 & 0.00 \\
& LIBERO-goal & all-layer & Prefill no image + generation no text & 200 & 0.00 \\
\cmidrule(lr){2-6}
& LIBERO-object & all-layer & Baseline & 200 & 74.00 \\
& LIBERO-object & all-layer & Generation drop newline & 200 & 71.50 \\
& LIBERO-object & all-layer & Generation drop prompt, keep newline & 200 & 0.00 \\
& LIBERO-object & all-layer & Generation no image & 200 & 32.50 \\
& LIBERO-object & all-layer & Generation no text & 200 & 0.00 \\
& LIBERO-object & all-layer & Prefill no image & 200 & 0.00 \\
& LIBERO-object & all-layer & Prefill no image + generation no image & 200 & 0.00 \\
& LIBERO-object & all-layer & Prefill no image + generation no text & 200 & 0.00 \\
\cmidrule(lr){2-6}
& LIBERO-spatial & all-layer & Baseline & 200 & 77.00 \\
& LIBERO-spatial & all-layer & Generation drop newline & 200 & 80.00 \\
& LIBERO-spatial & all-layer & Generation drop prompt, keep newline & 200 & 0.00 \\
& LIBERO-spatial & all-layer & Generation no image & 200 & 44.00 \\
& LIBERO-spatial & all-layer & Generation no text & 200 & 0.00 \\
& LIBERO-spatial & all-layer & Prefill no image & 200 & 0.00 \\
& LIBERO-spatial & all-layer & Prefill no image + generation no image & 200 & 0.00 \\
& LIBERO-spatial & all-layer & Prefill no image + generation no text & 200 & 0.00 \\
\bottomrule
\end{tabular}
\caption{Detailed attention knockout success rates ($\%$) across LIBERO suites. Each row corresponds to an observed result from the evaluation logs, avoiding artificial empty cells from crossing non-identical protocols. The 0410 LIBERO-goal/object/spatial rows report matched all-layer interventions, while LIBERO-10 rows include the available global and phase-specific all-layer protocol; $\pifive$ LIBERO-10 combo rows are the all-layer combo results reported by the window-7 analysis.}
\label{tab:knockout_summary}
\end{table*}

\begin{table*}[ht!]
\centering
\scriptsize
\setlength{\tabcolsep}{3.5pt}
\begin{tabular}{lllcccc}
\toprule
Model & Dataset & Layer-wise intervention & Mean SR & Worst layer & Worst SR & Worst drop \\
\midrule
$\pifive$ & LIBERO-10 & Prefill no V--L & 92.83 & L5 & 90.00 & -3.00 \\
$\pifive$ & LIBERO-10 & Generation no text & 92.67 & L11 & 91.00 & -2.00 \\
$\pifive$ & LIBERO-10 & Generation no image & 91.47 & L14 & 74.50 & -18.50 \\
$\pifive$ & LIBERO-10 & Prefill no V--L + generation no text & 92.89 & L7 & 89.50 & -3.50 \\
$\pifive$ & LIBERO-10 & Prefill no V--L + generation no image & 91.28 & L14 & 65.50 & -27.50 \\
\midrule
$\pifive$ & LIBERO-goal & Generation drop BOS+newline & 97.08 & L0 & 95.00 & -1.00 \\
$\pifive$ & LIBERO-goal & Generation drop instruction & 96.75 & L1 & 95.50 & -0.50 \\
$\pifive$ & LIBERO-goal & Generation keep BOS+newline only & 69.11 & L13 & 14.50 & -81.50 \\
$\pifive$ & LIBERO-goal & Generation no image & 79.92 & L13 & 34.50 & -61.50 \\
$\pifive$ & LIBERO-goal & Generation no text & 96.67 & L9 & 93.50 & -2.50 \\
$\pifive$ & LIBERO-goal & Prefill no V--L & 81.64 & L6 & 28.00 & -68.00 \\
$\pifive$ & LIBERO-goal & Prefill no V--L + generation no image & 60.64 & L11 & 21.50 & -74.50 \\
$\pifive$ & LIBERO-goal & Prefill no V--L + generation no text & 80.81 & L6 & 23.00 & -73.00 \\
\midrule
$\pifive$ & LIBERO-object & Generation drop BOS+newline & 98.86 & L9 & 97.50 & -1.00 \\
$\pifive$ & LIBERO-object & Generation drop instruction & 98.72 & L5 & 97.50 & -1.00 \\
$\pifive$ & LIBERO-object & Generation keep BOS+newline only & 72.89 & L11 & 10.50 & -88.00 \\
$\pifive$ & LIBERO-object & Generation no image & 85.25 & L11 & 43.00 & -55.50 \\
$\pifive$ & LIBERO-object & Generation no text & 98.78 & L1 & 97.50 & -1.00 \\
$\pifive$ & LIBERO-object & Prefill no V--L & 96.03 & L5 & 84.00 & -14.50 \\
$\pifive$ & LIBERO-object & Prefill no V--L + generation no image & 77.25 & L11 & 10.50 & -88.00 \\
$\pifive$ & LIBERO-object & Prefill no V--L + generation no text & 96.06 & L4 & 85.00 & -13.50 \\
\midrule
$\pifive$ & LIBERO-spatial & Generation drop BOS+newline & 99.08 & L5 & 97.50 & -1.00 \\
$\pifive$ & LIBERO-spatial & Generation drop instruction & 98.53 & L17 & 95.50 & -3.00 \\
$\pifive$ & LIBERO-spatial & Generation keep BOS+newline only & 70.58 & L13 & 7.50 & -91.00 \\
$\pifive$ & LIBERO-spatial & Generation no image & 79.14 & L13 & 33.00 & -65.50 \\
$\pifive$ & LIBERO-spatial & Generation no text & 98.64 & L0 & 96.50 & -2.00 \\
$\pifive$ & LIBERO-spatial & Prefill no V--L & 94.86 & L6 & 81.50 & -17.00 \\
$\pifive$ & LIBERO-spatial & Prefill no V--L + generation no image & 71.17 & L11 & 8.00 & -90.50 \\
$\pifive$ & LIBERO-spatial & Prefill no V--L + generation no text & 94.58 & L5 & 82.50 & -16.00 \\
\midrule
OpenVLA & LIBERO-10 & Generation drop newline & 52.88 & L5 & 44.50 & -13.50 \\
OpenVLA & LIBERO-10 & Generation drop prompt, keep newline & 51.80 & L15 & 38.50 & -19.50 \\
OpenVLA & LIBERO-10 & Generation no text & 50.89 & L15 & 35.00 & -23.00 \\
OpenVLA & LIBERO-10 & Generation no image & 53.16 & L10 & 45.50 & -12.50 \\
OpenVLA & LIBERO-10 & Prefill no image & 51.09 & L11 & 25.50 & -32.50 \\
OpenVLA & LIBERO-10 & Prefill no image + generation no text & 48.76 & L15 & 22.50 & -35.50 \\
\midrule
OpenVLA & LIBERO-goal & Generation drop newline & 75.58 & L13 & 70.00 & -9.50 \\
OpenVLA & LIBERO-goal & Generation drop prompt, keep newline & 45.75 & L2 & 0.00 & -79.50 \\
OpenVLA & LIBERO-goal & Generation no image & 67.72 & L12 & 49.00 & -30.50 \\
OpenVLA & LIBERO-goal & Generation no text & 42.69 & L2 & 0.00 & -79.50 \\
OpenVLA & LIBERO-goal & Prefill no image & 45.73 & L11 & 0.00 & -79.50 \\
OpenVLA & LIBERO-goal & Prefill no image + generation no image & 45.69 & L11 & 0.00 & -79.50 \\
OpenVLA & LIBERO-goal & Prefill no image + generation no text & 34.61 & L2 & 0.00 & -79.50 \\
\midrule
OpenVLA & LIBERO-object & Generation drop newline & 74.06 & L28 & 68.50 & -5.50 \\
OpenVLA & LIBERO-object & Generation drop prompt, keep newline & 49.98 & L2 & 0.00 & -74.00 \\
OpenVLA & LIBERO-object & Generation no image & 68.53 & L10 & 53.00 & -21.00 \\
OpenVLA & LIBERO-object & Generation no text & 47.33 & L2 & 0.00 & -74.00 \\
OpenVLA & LIBERO-object & Prefill no image & 43.44 & L2 & 0.00 & -74.00 \\
OpenVLA & LIBERO-object & Prefill no image + generation no image & 43.44 & L2 & 0.00 & -74.00 \\
OpenVLA & LIBERO-object & Prefill no image + generation no text & 33.66 & L1 & 0.00 & -74.00 \\
\midrule
OpenVLA & LIBERO-spatial & Generation drop newline & 78.28 & L6 & 74.50 & -2.50 \\
OpenVLA & LIBERO-spatial & Generation drop prompt, keep newline & 49.25 & L2 & 0.00 & -77.00 \\
OpenVLA & LIBERO-spatial & Generation no image & 74.09 & L13 & 63.00 & -14.00 \\
OpenVLA & LIBERO-spatial & Generation no text & 46.47 & L2 & 0.00 & -77.00 \\
OpenVLA & LIBERO-spatial & Prefill no image & 49.16 & L12 & 0.00 & -77.00 \\
OpenVLA & LIBERO-spatial & Prefill no image + generation no image & 49.89 & L3 & 0.50 & -76.50 \\
OpenVLA & LIBERO-spatial & Prefill no image + generation no text & 36.72 & L1 & 0.00 & -77.00 \\
\bottomrule
\end{tabular}
\caption{Unified layer-wise knockout summary across models and LIBERO suites. Mean SR averages success rates across scanned layers; Worst SR and Worst drop report the most damaging layer-wise intervention relative to the corresponding layer-wise baseline. The $\pifive$ LIBERO-10 scan covers L0--L17; the OpenVLA LIBERO-10 scan covers L0--L31 except for one missing terminal-layer record in the combined prefill-image/generation-text setting.}
\label{tab:layerwise_knockout_summary}
\end{table*}

\subsubsection{Attention Knockout}
As illustrated in Figure~\ref{fig:all_layers_knockout} and Table~\ref{tab:knockout_summary}, we observe distinct modality dependencies across models and inference stages. For $\pifive$, the matched 0410 LIBERO-goal/object/spatial suites show that action generation relies heavily on visual information once the context has been formed. Removing the generation-time image pathway reduces success to 4.00\% on LIBERO-goal and to 0.00\% on both LIBERO-object and LIBERO-spatial. Keeping only BOS and newline tokens during generation is similarly destructive, showing that these structural tokens cannot substitute for the missing visual stream. In contrast, removing generation-time text alone on the same three suites retains high success, with \texttt{generation\_no\_text} staying above 96.00\%. This does not mean that language is irrelevant. Rather, it indicates that, in these suites, task information can be incorporated during the prefill stage and reused during decoding, whereas the online action bottleneck is dominated by visual evidence.

The prefill interventions sharpen this interpretation. Blocking visual-language interaction before action decoding reduces $\pifive$ success to 11.50\% on LIBERO-goal, 71.50\% on LIBERO-object, and 76.25\% on LIBERO-spatial, and combining prefill no-V--L with generation no-image collapses all three suites to 0.00\%. Thus, $\pifive$ should not be described as simply ignoring language. A more precise conclusion, following the two-stage knockout design, is that language contributes to the construction of the prefilled multimodal state, while the most fragile decoding-time pathway is the visual-to-action route. LIBERO-10 provides a complementary stress test: $\pifive$ retains 86.20\% under generation no-image and 82.80\% under prefill no-V--L, but drops to 0.40\% under global no-text and 0.00\% under global no-V--L. This shows that global textual availability can remain necessary under stronger all-layer removal even when single-stage or single-layer text removal appears redundant.

The layer-wise scan in Table~\ref{tab:layerwise_knockout_summary} further localizes the bottleneck. For $\pifive$, the strongest visual failures consistently appear in middle-to-late layers: LIBERO-10 reaches its worst visual-combination drop at L14, while the 0410 suites expose severe drops around L11--L13 under generation no-image or prefill no-V--L plus generation no-image. By contrast, layer-wise generation no-text is close to baseline for $\pifive$, with only a 2.00-point worst-layer drop on LIBERO-10 and similarly small drops on the 0410 suites. Therefore, \ul{$\pifive$ concentrates the decisive visual information for action generation in a middle-to-late bottleneck, while textual information is more distributed and redundant at the single-layer decoding interface.}

Compared with $\pifive$, OpenVLA exhibits a different behavior. Across LIBERO-goal, LIBERO-object, and LIBERO-spatial, removing generation-time text reduces success to 0.00\%, and dropping the prompt while keeping only the newline token also reduces success to 0.00\%. Prefill image removal is equally destructive, producing 0.00\% on all three suites. On LIBERO-10, OpenVLA also collapses under generation no-text, generation no-image, prefill no-image, global no-image, global no-text, and global no-V--L, while prefill no-text retains 47.40\%. These results indicate that OpenVLA depends strongly on both prompt-region access during generation and visual grounding during prefill. However, because the prompt region contains both semantic instruction words and template tokens such as ``In'' and ``Out'', knockout alone should be interpreted as evidence of functional prompt-pathway dependence rather than definitive proof of compositional semantic grounding.

Finally, layer-wise knockout shows that critical information is more broadly distributed in OpenVLA than in $\pifive$. On the 0410 suites, generation no-text and prompt-drop interventions reach their worst failures at early layers such as L2, often reducing success to 0.00\%. Prefill-image interventions also reveal severe vulnerable layers, while generation-image removal is damaging but less uniformly catastrophic, retaining 16.00\%--44.00\% in the all-layer 0410 setting. Together with the CKA evidence that OpenVLA preserves textual geometry while concentrating robot-domain fusion near terminal layers, these results suggest that OpenVLA maintains a functionally critical prompt pathway, but its semantic flexibility must be tested by input-editing experiments rather than inferred from knockout alone.

\begin{table}[h!]
\begin{tcolorbox}[
    colback=blue!5!white,
    colframe=black,
    width=\linewidth,
    boxrule=0.5pt,
    sharp corners,
    fonttitle=\bfseries,
    coltitle=black,
    before skip=5pt,
    after skip=5pt,
    boxsep=0pt,
    left=5pt, right=5pt, top=5pt, bottom=5pt
]
\noindent \textbf{\textcolor{black}{Summary.}} \small

For action generation, $\pifive$ concentrates the most fragile visual control signal in middle-to-late layers, especially around L11--L14, forming a key visual-to-action bottleneck. Textual information is not absent, but its causal role is more distributed and stage-dependent: it can be necessary under global or prefill-level removal while remaining redundant under single-layer generation-time text knockout. In contrast, OpenVLA is strongly dependent on prompt-region tokens during generation and on image access during prefill, with critical effects spread across broader layer ranges. Attention knockout therefore shows that the two models achieve control through different execution channels: $\pifive$ routes a prefilled multimodal state through a visual-action bottleneck, whereas OpenVLA relies on a prompt-region pathway whose true semantic flexibility must be evaluated by editing probes.
\end{tcolorbox}
\end{table}

==> sections/exp.tex <==
\section{Empirical Analysis} \label{sec:empirical}

\input{sections/cka_knockout}

\subsection{Manifestation of Execution Shortcuts}
\label{subsec:shortcut_manifestation}

This section addresses \textit{\textbf{RQ3:} How do representation and intervention evidence manifest as concrete visual shortcuts and semantic instruction-following failures?} After analyzing representation dynamics and causal control pathways, we further examine whether these internal findings correspond to observable behavior. Specifically, we use attention IoU and visualization to quantify where action attention is routed during rollouts, visual patch masking to measure dependence on specific image regions, and input editing to test whether visual-layout or language-semantic changes redirect the policy. Together, these analyses evaluate whether the identified execution pathways correspond to dependencies on actionable regions, active subtask objects, effector-centered views, and prompt-template cues.

\subsubsection{Attention IoU and Attention Patterns}
\begin{table*}[t]
\centering
\small
\begin{tabular}{llccc}
\toprule
Model / metric & Region or quantity & Phase 1 & Phase 2 & Full rollout \\
\midrule
\multirow{3}{*}{$\pifive$ localization}
& Task-02 Top-10 patch IoU & 0.2961 $\pm$ 0.0273 & 0.2660 $\pm$ 0.0375 & 0.2580 \\
& Task-02 peak hit & 0.6200 & 0.6186 & 0.6073 \\
& LIBERO-10 macro Top-10 patch IoU / peak hit & \multicolumn{3}{c}{0.2197 $\pm$ 0.0244 / 0.6588 $\pm$ 0.1907} \\
\midrule
\multirow{2}{*}{OpenVLA Top-10 patch IoU}
& Gripper & 0.1623 & 0.1420 & 0.1522 \\
& Task objects & 0.0601 & 0.0576 & 0.0589 \\
\bottomrule
\end{tabular}
\caption{IoU-based attention localization during closed-loop LIBERO rollouts. Top-10 patch IoU measures the overlap between the top 10\% action-attended visual patches and simulator-derived instance masks on a $16\times16$ grid. For $\pifive$, we report both the representative stove-and-moka trajectory (Task-02) and the macro average over ten successful LIBERO-10 rollouts. For OpenVLA, we report the available fine-tuned rollout summaries.}
\label{tab:attention_grounding}
\end{table*}

\begin{figure*}[t]
    \centering
    \begin{subfigure}{0.68\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figs/pi05_iou_rollout_curve.pdf}
        \caption{$\pifive$ step-wise IoU on the stove-and-moka trajectory.}
        \label{fig:pi05_iou_curve}
    \end{subfigure}
    
    \vspace{0.5em}
    \begin{subfigure}{0.98\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figs/openvla_iou_phase_by_task.pdf}
        \caption{OpenVLA phase-wise IoU across LIBERO-10 tasks.}
        \label{fig:openvla_iou_curve}
    \end{subfigure}
    \caption{IoU curves for attention localization. The top panel tracks $\pifive$ Top-10 patch IoU over rollout steps, with the dotted line marking the transition from the stove-knob phase to the moka-pot phase. The bottom panel shows OpenVLA phase-wise mean IoU between top-attended patches and task objects across the available LIBERO-10 rollout summaries.}
    \label{fig:attention_iou_curves}
\end{figure*}

\begin{table*}[t]
\centering
\small
\begin{tabular}{llccc}
\toprule
Model / analysis & Region or quantity & Phase 1 & Phase 2 & Full rollout \\
\midrule
\multirow{5}{*}{$\pifive$ attention mass}
& GT union & 0.6566 & 0.6373 & 0.6469 \\
& Gripper & 0.2128 & 0.1594 & 0.1860 \\
& Robot arm & 0.1756 & 0.1983 & 0.1870 \\
& Manipulated object & 0.1343 & 0.1316 & 0.1329 \\
& Receptacle / affordance & 0.1339 & 0.1480 & 0.1409 \\
\midrule
\multirow{4}{*}{$\pifive$ stage tracking}
& Successful rollouts / analyzed steps & \multicolumn{3}{c}{10 / 2632} \\
& Mean GT-union mass across tasks & \multicolumn{3}{c}{0.6469 $\pm$ 0.0187} \\
& Mean subtask focus-set mass & \multicolumn{3}{c}{0.2224} \\
& Active-object advantage over next-stage object & \multicolumn{3}{c}{0.0610 (max 0.1067)} \\
\midrule
OpenVLA rollout evidence & Pretrained / fine-tuned success & \multicolumn{3}{c}{0 / 50 \quad vs. \quad 31 / 50} \\
\bottomrule
\end{tabular}
\caption{Attention-mass and rollout-stage statistics from the supporting analyses. Unlike Top-10 patch IoU, attention mass preserves the continuous action-to-image heatmap and reports the fraction of total attention assigned to each simulator-derived region.}
\label{tab:attention_stage}
\end{table*}

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.78\textwidth]{figs/pi05_attention_mass_decomposition.pdf}
    \caption{$\pifive$ action-to-image attention mass by simulator region. Error bars denote the standard deviation across ten successful LIBERO-10 rollouts.}
    \label{fig:pi05_attention_mass_decomp}
\end{figure*}

\begin{table*}[t]
\centering
\small
\begin{tabular}{p{0.18\textwidth}p{0.34\textwidth}p{0.40\textwidth}}
\toprule
$\pifive$ evidence & Quantitative observation & Interpretation \\
\midrule
Rollout contrast & Pretrained model: 0\% success and 520-step failures; fine-tuned model: 100\% success and 231-step completion on the representative rollout. & Finetuning changes attention from diffuse scene reading to executable manipulation tracking. \\
View allocation & In the layer-wise attention summary, action queries allocate roughly 19\% mass to the wrist view and 9\% to the agent view, after accounting for the BOS-dominated text sink. & $\pifive$ uses the closer manipulation view more strongly, consistent with reliance on local contact and affordance cues. \\
Layer routing & Early layers L0--L3 mainly perform coarse input reading; visual use increases through L8--L13; L14 shows the strongest image--action coupling; L15--L17 mainly propagate action information. & The visual grounding signal is not monotonically stronger in later layers, but peaks near the layer where image removal is most damaging. \\
Attention sink & BOS self-attention reaches 0.81, and query groups send approximately 28--45\% of their mass to BOS; other text tokens allocate about 70\% mass within the text/BOS loop and only about 28\% to images. & Raw text attention can overstate semantic language use; special tokens must be separated before interpreting instruction grounding. \\
Action slots & The ten action slots have nearly symmetric attention distributions under bidirectional self-attention. & $\pifive$ encodes the action chunk as a coupled block, so visual routing affects the whole action segment rather than a single scalar action. \\
\bottomrule
\end{tabular}
\caption{Additional $\pifive$ attention-routing evidence from the layer-wise visualization analysis. These statistics complement the IoU and mass results by explaining where the attention signal is routed inside the transformer.}
\label{tab:pi05_attention_routing}
\end{table*}

We analyze attention distributions during real closed-loop rollouts in LIBERO, starting with an IoU-based localization test before examining continuous attention mass, model-specific routing statistics, and qualitative visualizations. Attention visualization provides an intuitive view of information flow, while Attention IoU turns action-attention localization into a measurable grounding probe. We use the instruction \textit{``Turn on the stove and put the moka pot on it.''} as a representative sequential manipulation case, and complement this case study with mask statistics across ten successful $\pifive$ LIBERO-10 rollouts. For action-to-image and action-to-text attention, we extract attention maps from the final denoising step and average over action slots to obtain a stable estimate. To test whether the most attended visual patches are spatially grounded, we render simulator instance masks on the same $16\times16$ patch grid. We report three complementary localization metrics: Top-10 patch IoU, which keeps only the top 10\% highest-attention patches; attention mass inside a mask, which preserves the full continuous heatmap; and peak-hit rate, which checks whether the single maximum-attention patch lies inside the ground-truth mask.

As shown in Table~\ref{tab:attention_grounding} and Figure~\ref{fig:attention_iou_curves}, the IoU experiment provides a conservative localization view because it keeps only the highest-attention patches. In the stove-and-moka trajectory, $\pifive$ obtains a Top-10 patch IoU of 0.2961 $\pm$ 0.0273 in the first phase, where the policy must operate around the stove knob, and 0.2660 $\pm$ 0.0375 in the second phase, where the policy shifts toward the moka pot and placement region. The corresponding peak-hit rates remain stable at 0.6200 and 0.6186, respectively. Across the ten LIBERO-10 rollouts, the macro Top-10 patch IoU is 0.2197 $\pm$ 0.0244, while the peak-hit rate is 0.6588 $\pm$ 0.1907. These values indicate that \ul{the strongest attention patches are not arbitrary image saliency, but frequently intersect the simulator-defined regions needed for manipulation.} More importantly, the phase-wise object analysis reveals that attention follows the temporal decomposition of the instruction rather than only the globally salient object. Averaged across tasks, the first manipulated object receives more mass in the first segment than in the second segment by 0.0572, while the second manipulated object receives more mass in the second segment by 0.0648. OpenVLA shows a different localization profile in the available rollout summaries: its Top-10 attended patches overlap the gripper mask more strongly than task-object masks, with full-rollout IoU means of 0.1522 and 0.0589. Together with the rollout summary in Table~\ref{tab:attention_stage}, where pretrained OpenVLA succeeds in 0/50 available rollouts while the fine-tuned model succeeds in 31/50, this suggests that the fine-tuned policy acquires a more executable but also more effector-centered attention pattern.

We next measure continuous attention mass, which avoids discarding the non-top patches and therefore complements the thresholded IoU view. Given an action-to-image attention matrix $A \in \mathbb{R}^{N_q \times N_k}$, a set of action-query tokens $Q$, and a simulator mask $M$, we compute:
\begin{equation}
\mathrm{Mass}(M) = \frac{\sum_{j \in M} \bar{A}_{j}}{\sum_{j} \bar{A}_{j}}, \quad
\bar{A}_{j}=\frac{1}{|Q|}\sum_{i\in Q} A_{ij},
\end{equation}
where $\bar{A}_{j}$ is the action-averaged attention assigned to image patch $j$. Table~\ref{tab:attention_stage} and Figure~\ref{fig:pi05_attention_mass_decomp} show that $\pifive$ assigns 0.6469 attention mass to the ground-truth union masks on average, with similar values in the first and second task phases (0.6566 and 0.6373). The role-wise decomposition further reveals a temporal shift. Gripper mass decreases from 0.2128 to 0.1594, while robot-arm and receptacle/affordance mass increase from 0.1756 to 0.1983 and from 0.1339 to 0.1480, respectively. This shift is consistent with the policy moving from initial contact and knob manipulation to transport, placement, or closure. The manipulated-object mass is more stable at the coarse role level, but the slot-specific analysis shows that the identity of the attended object changes with the subtask: for example, in the stove-and-moka trajectory, stove mass is larger in phase 1 (0.1750 versus 0.1228), whereas moka-pot mass is larger in phase 2 (0.0915 versus 0.0389). Thus, the continuous heatmap leads to the same conclusion as the IoU analysis, but with a more detailed view of how the policy distributes attention among the gripper, robot body, currently manipulated object, and downstream affordance.

The $\pifive$ routing statistics in Table~\ref{tab:pi05_attention_routing} connect this rollout-level grounding to the layer-wise intervention results in Section~\ref{subsec:attention_knockout}. The pretrained $\pifive$ rollout fails for the full 520-step horizon, whereas the fine-tuned rollout succeeds in 231 steps, and the qualitative attention maps show that finetuning changes the policy from diffuse scene attention to stage-specific focus on the gripper, stove knob, and moka-pot handle. However, this does not imply robust compositional semantic grounding. After separating special-token effects, action queries still allocate roughly twice as much attention to the wrist view as to the agent view (19\% versus 9\%), indicating a local manipulation-view shortcut. The same layer-wise summary reports that L14 is where image--action coupling is strongest, matching the knockout observation that generation-time image removal around the middle-to-late layers produces the largest success drop for $\pifive$. Thus, attention visualization not only illustrates where the model attends, but also helps explain why a narrow visual pathway can dominate action generation even when the language prompt remains available.

\begin{figure*}[ht!]
    \centering
    \includegraphics[width=\textwidth]{figs/attn_vis.pdf}
    \caption{Visualization of action-to-image attention at different timesteps (top to bottom: steps 0, 30, 60, 100, and 250). The left two columns show the agent view, while the right two columns show the wrist view.}
    \label{fig:a2i}
\end{figure*}
\begin{figure*}[ht!]
    \centering
    \includegraphics[width=\textwidth]{figs/attn_vis_1.pdf}
    \caption{Visualization of action-to-text attention at different timesteps (top to bottom: steps 0, 30, 60, 100, and 250).}
    \label{fig:a2i_1}
\end{figure*}
\begin{figure*}[ht!]
    \centering
    \includegraphics[width=\textwidth]{figs/attn_vis_4.pdf}
    \caption{Visualization of layer-wise modality attention (left: step 30, right: step 150) (Top: pretrained, bottom: fine-tuned).}
    \label{fig:a2i_4}
\end{figure*}

The visualizations in Figures~\ref{fig:a2i}--\ref{fig:a2i_4} explain the preceding statistics at the level of individual rollout behavior. Figure~\ref{fig:a2i} shows that action-to-image attention initially covers the gripper and stove knob; by the middle of the trajectory, it follows the ``turn on the stove'' subtask; and after the subtask boundary, it shifts toward the moka pot and placement region. Figure~\ref{fig:a2i_1} further shows that action-to-text attention changes with the task stage, but the language signal remains coarser than the visual signal: the fine-tuned model attends to action-related tokens such as ``turn'' early in the rollout and later increases attention to ``moka'', ``pot'', and ``put'', whereas the pretrained model remains less adaptive. This textual selectivity should be interpreted carefully because Table~\ref{tab:pi05_attention_routing} shows a strong BOS/newline attention sink; before special-token separation, text attention can appear large even when much of it is absorbed by formatting tokens rather than instruction semantics. Finally, the layer-wise modality attention in Figure~\ref{fig:a2i_4} shows that both pretrained and fine-tuned models allocate more attention to visual inputs than to language, with the fine-tuned model further amplifying visual attention around the action phase. This is consistent with the knockout result that $\pifive$ is highly sensitive to generation-time visual removal, but it also clarifies the behavioral form of this dependence: visual information is used as a stage-aware execution signal, while language provides a comparatively sparse task scaffold. Importantly, this attention evidence should not be interpreted as sufficient proof of robust semantic grounding. It instead shows how the execution channels identified by knockout appear in rollout behavior: $\pifive$ tracks task-relevant masks, active subtask objects, and wrist-view affordances, while OpenVLA concentrates more strongly on effector regions under the available patch-IoU view.

\subsubsection{Visual Patch Masking}
\input{tabs/patch_mask_1}
\input{tabs/patch_mask_2}
\input{tabs/patch_mask_3}
\input{tabs/patch_mask_goal}

In this experiment, we investigate the impact of visual perturbations by selectively masking specific regions of the visual input, including the target object, the gripper, the robot body, and the background. For each region, we apply three masking strategies: background-color replacement, uniform black masking, and mosaic masking. Tables~\ref{tab:mask1}, \ref{tab:mask2}, \ref{tab:mask3}, and \ref{tab:mask_goal} present the resulting success rates across LIBERO-10, LIBERO-Object, LIBERO-Spatial, and LIBERO-Goal. 

Across all settings, target-object masking causes the most severe performance degradation. On LIBERO-10, $\pifive$ drops from 75.00\% to 0.00\% under target background replacement, while OpenVLA drops from 52.33\% to 6.00\%. Similar collapses occur on LIBERO-Object ($\pifive$ drops from 95.60\% to 13.00\%), LIBERO-Spatial (95.80\% to 7.80\%), and LIBERO-Goal (80.00\% to 19.80\%). These results indicate that \ul{the target object provides a necessary visual anchor for action execution.}

Furthermore, the differential effect of the masking types reveals the nature of the visual information utilized by the policy. Background replacement is consistently more damaging than black or mosaic masking. For instance, on LIBERO-Object, target background replacement reduces $\pifive$ success to 13.00\%, whereas black and mosaic masking retain 61.60\% and 74.00\% success, respectively. This suggests that background replacement effectively removes both appearance and boundary cues, whereas black and mosaic masks preserve coarse shape or spatial structure. Gripper and robot masking exhibit a related pattern: on LIBERO-10, $\pifive$ drops to 8.40\% under gripper background replacement, but maintains 52.60\% and 53.20\% under black and mosaic masking. Therefore, \ul{the model relies not only on fine-grained object appearance but also on coarse spatial relationships between the target, gripper, and robot body.}

\subsubsection{Input Editing}
\input{tabs/text_edit}

% \begin{figure}[ht!]
%     \centering
%     \includegraphics[width=\columnwidth]{figs/image_edit.pdf}
%     \caption{Visualization of image editing examples.}
%     \label{fig:image_edit}
% \end{figure}

Finally, we evaluate whether the model dynamically follows controlled changes in image layout and language semantics.
% For image editing (Figure~\ref{fig:image_edit}), altering object positions causes an average performance drop of 16 points. 
The most significant degradation occurs in multi-object arrangements and overlapping-object scenarios. This indicates that the policy is sensitive to object position changes, particularly when the edited scene disrupts the spatial relations required for manipulation. 

For text editing, Table~\ref{tab:text_edit} serves as a targeted case study rather than a comprehensive behavioral benchmark. Replacing target objects in the instruction does not consistently redirect the model toward the edited target. For example, changing ``moka pot'' to ``frypan'' reduces success from 75\% to 30\%, and changing ``book'' to ``mug'' reduces success from 90\% to 30\%. However, other edits, such as replacing ``tomato sauce'' with ``ketchup'' or ``white mug'' with ``red mug,'' do not produce a consistent failure pattern. We interpret this probe as evidence of partial, edit-type-dependent semantic redirection. While the current editing experiment does not exhaustively classify whether each failed trajectory follows the original object, stops, or switches to a distractor, the overall result supports the VLA-Trace diagnosis: \ul{text exerts a non-negligible but limited influence on action execution, and the policy often remains biased toward the original visual-task configuration even when edited semantics dictate a behavioral shift.}

\begin{table}[h!]
\begin{tcolorbox}[
    colback=blue!5!white,
    colframe=black,
    width=\linewidth,
    boxrule=0.5pt,
    sharp corners,
    fonttitle=\bfseries,
    coltitle=black,
    before skip=5pt,
    after skip=5pt,
    boxsep=0pt,
    left=5pt, right=5pt, top=5pt, bottom=5pt
]
\noindent \textbf{\textcolor{black}{Summary.}} \small

Attention IoU, visualization, visual patch masking, and input editing collectively demonstrate how internal execution channels manifest in observable behavior. $\pifive$ attends to actionable masks, active subtask objects, wrist-view affordances, and a middle-layer image--action routing bottleneck, while also exhibiting special-token attention sinks that caution against naive interpretations of language attention. OpenVLA displays a more effector-centered IoU pattern and stronger prompt-region dependence under knockout. Together, the vulnerability to target-object and gripper perturbations, the partial adherence to text edits, and the stage-aware attention shifts support our core conclusion: current VLA policies rely heavily on task-specialized visual-spatial shortcuts rather than robust, compositional semantic grounding.
\end{tcolorbox}
\end{table}


==> tabs/all_layer_knockout.tex <==
\begin{table*}[ht!]
\centering
\scriptsize
\setlength{\tabcolsep}{3.5pt}
\begin{tabular}{llllcc}
\toprule
Model & Dataset & Protocol & Intervention & Episodes & SR \\
\midrule
\multirow{38}{*}{$\pifive$}
& LIBERO-10 & baseline & Baseline & 200 & 91.20 \\
& LIBERO-10 & phase & Generation no image & 200 & 86.20 \\
& LIBERO-10 & phase & Generation no text & 200 & 1.40 \\
& LIBERO-10 & phase & Prefill no V--L & 200 & 82.80 \\
& LIBERO-10 & phase & Prefill no image & 200 & 81.20 \\
& LIBERO-10 & phase & Prefill no text & 200 & 80.60 \\
& LIBERO-10 & global & Global no image & 200 & 47.80 \\
& LIBERO-10 & global & Global no text & 200 & 0.40 \\
& LIBERO-10 & global & Global no V--L & 200 & 0.00 \\
& LIBERO-10 & all-layer combo & Prefill no V--L + generation no image & 200 & 0.00 \\
& LIBERO-10 & all-layer combo & Prefill no V--L + generation no text & 200 & 73.50 \\
\cmidrule(lr){2-6}
& LIBERO-goal & all-layer & Baseline & 200 & 97.00 \\
& LIBERO-goal & all-layer & Generation drop BOS+newline & 200 & 97.50 \\
& LIBERO-goal & all-layer & Generation drop instruction & 200 & 97.00 \\
& LIBERO-goal & all-layer & Generation keep BOS+newline only & 200 & 1.50 \\
& LIBERO-goal & all-layer & Generation no image & 200 & 4.00 \\
& LIBERO-goal & all-layer & Generation no text & 200 & 96.50 \\
& LIBERO-goal & all-layer & Prefill no V--L & 200 & 11.50 \\
& LIBERO-goal & all-layer & Prefill no V--L + generation no image & 200 & 0.00 \\
& LIBERO-goal & all-layer & Prefill no V--L + generation no text & 200 & 11.75 \\
\cmidrule(lr){2-6}
& LIBERO-object & all-layer & Baseline & 200 & 98.33 \\
& LIBERO-object & all-layer & Generation drop BOS+newline & 200 & 99.50 \\
& LIBERO-object & all-layer & Generation drop instruction & 200 & 99.50 \\
& LIBERO-object & all-layer & Generation keep BOS+newline only & 200 & 0.00 \\
& LIBERO-object & all-layer & Generation no image & 200 & 0.00 \\
& LIBERO-object & all-layer & Generation no text & 200 & 98.00 \\
& LIBERO-object & all-layer & Prefill no V--L & 200 & 71.50 \\
& LIBERO-object & all-layer & Prefill no V--L + generation no image & 200 & 0.00 \\
& LIBERO-object & all-layer & Prefill no V--L + generation no text & 200 & 46.00 \\
\cmidrule(lr){2-6}
& LIBERO-spatial & all-layer & Baseline & 200 & 99.00 \\
& LIBERO-spatial & all-layer & Generation drop BOS+newline & 200 & 99.00 \\
& LIBERO-spatial & all-layer & Generation drop instruction & 200 & 100.00 \\
& LIBERO-spatial & all-layer & Generation keep BOS+newline only & 200 & 0.00 \\
& LIBERO-spatial & all-layer & Generation no image & 200 & 0.00 \\
& LIBERO-spatial & all-layer & Generation no text & 200 & 99.00 \\
& LIBERO-spatial & all-layer & Prefill no V--L & 200 & 76.25 \\
& LIBERO-spatial & all-layer & Prefill no V--L + generation no image & 200 & 0.00 \\
& LIBERO-spatial & all-layer & Prefill no V--L + generation no text & 200 & 70.67 \\
\midrule
\multirow{32}{*}{OpenVLA}
& LIBERO-10 & baseline & Baseline & 200 & 56.80 \\
& LIBERO-10 & phase & Generation no image & 200 & 1.00 \\
& LIBERO-10 & phase & Generation no text & 200 & 0.00 \\
& LIBERO-10 & phase & Prefill no image & 200 & 0.00 \\
& LIBERO-10 & phase & Prefill no text & 200 & 47.40 \\
& LIBERO-10 & global & Global no image & 200 & 0.00 \\
& LIBERO-10 & global & Global no text & 200 & 0.00 \\
& LIBERO-10 & global & Global no V--L & 200 & 0.00 \\
\cmidrule(lr){2-6}
& LIBERO-goal & all-layer & Baseline & 200 & 77.25 \\
& LIBERO-goal & all-layer & Generation drop newline & 200 & 75.50 \\
& LIBERO-goal & all-layer & Generation drop prompt, keep newline & 200 & 0.00 \\
& LIBERO-goal & all-layer & Generation no image & 200 & 16.00 \\
& LIBERO-goal & all-layer & Generation no text & 200 & 0.00 \\
& LIBERO-goal & all-layer & Prefill no image & 200 & 0.00 \\
& LIBERO-goal & all-layer & Prefill no image + generation no image & 200 & 0.00 \\
& LIBERO-goal & all-layer & Prefill no image + generation no text & 200 & 0.00 \\
\cmidrule(lr){2-6}
& LIBERO-object & all-layer & Baseline & 200 & 74.00 \\
& LIBERO-object & all-layer & Generation drop newline & 200 & 71.50 \\
& LIBERO-object & all-layer & Generation drop prompt, keep newline & 200 & 0.00 \\
& LIBERO-object & all-layer & Generation no image & 200 & 32.50 \\
& LIBERO-object & all-layer & Generation no text & 200 & 0.00 \\
& LIBERO-object & all-layer & Prefill no image & 200 & 0.00 \\
& LIBERO-object & all-layer & Prefill no image + generation no image & 200 & 0.00 \\
& LIBERO-object & all-layer & Prefill no image + generation no text & 200 & 0.00 \\
\cmidrule(lr){2-6}
& LIBERO-spatial & all-layer & Baseline & 200 & 77.00 \\
& LIBERO-spatial & all-layer & Generation drop newline & 200 & 80.00 \\
& LIBERO-spatial & all-layer & Generation drop prompt, keep newline & 200 & 0.00 \\
& LIBERO-spatial & all-layer & Generation no image & 200 & 44.00 \\
& LIBERO-spatial & all-layer & Generation no text & 200 & 0.00 \\
& LIBERO-spatial & all-layer & Prefill no image & 200 & 0.00 \\
& LIBERO-spatial & all-layer & Prefill no image + generation no image & 200 & 0.00 \\
& LIBERO-spatial & all-layer & Prefill no image + generation no text & 200 & 0.00 \\
\bottomrule
\end{tabular}
\caption{Detailed attention knockout success rates ($\%$) across LIBERO suites. Each row corresponds to an observed result from the evaluation logs, avoiding artificial empty cells from crossing non-identical protocols. The 0410 LIBERO-goal/object/spatial rows report matched all-layer interventions, while LIBERO-10 rows include the available global and phase-specific all-layer protocol; $\pifive$ LIBERO-10 combo rows are the all-layer combo results reported by the window-7 analysis.}
\label{tab:knockout_summary}
\end{table*}

==> tabs/attention_knockout_all_layers_summary.tex <==
\begin{table*}[t]
\centering
\scriptsize
\setlength{\tabcolsep}{4pt}
\begin{tabular}{llccccc}
\toprule
Model & Setting & LIBERO-10 & Goal & Spatial & Object & Avg. \\
\midrule
\multirow{9}{*}{$\pifive$}
& Baseline & 93.5 (0.0) & 98.0 (0.0) & 99.3 (0.0) & 98.3 (0.0) & 97.3 (0.0) \\
& Gen: drop BOS+newline & 92.5 (-1.0) & 97.5 (-0.5) & 99.0 (-0.3) & 99.5 (+1.3) & 97.1 (-0.1) \\
& Gen: drop instruction & 94.5 (+1.0) & 97.0 (-1.0) & 100.0 (+0.8) & 99.5 (+1.3) & 97.8 (+0.5) \\
& Gen: keep BOS+newline only & 0.0 (-93.5) & 1.5 (-96.5) & 0.0 (-99.3) & 0.0 (-98.3) & 0.4 (-96.9) \\
& Gen: no image & 0.0 (-93.5) & 4.0 (-94.0) & 0.0 (-99.3) & 0.0 (-98.3) & 1.0 (-96.3) \\
& Gen: no text & 91.0 (-2.5) & 96.5 (-1.5) & 99.0 (-0.3) & 98.0 (-0.3) & 96.1 (-1.1) \\
& Prefill: no V--L & 82.0 (-11.5) & 11.5 (-86.5) & 76.3 (-23.0) & 71.5 (-26.8) & 60.3 (-36.9) \\
& Prefill no V--L + Gen no image & 0.0 (-93.5) & 0.0 (-98.0) & 0.0 (-99.3) & 0.0 (-98.3) & 0.0 (-97.3) \\
& Prefill no V--L + Gen no text & 74.0 (-19.5) & 11.5 (-86.5) & 70.3 (-29.0) & 46.0 (-52.3) & 50.4 (-46.8) \\
\midrule
\multirow{8}{*}{OpenVLA}
& Baseline & 58.5 (0.0) & 75.0 (0.0) & 77.0 (0.0) & 74.0 (0.0) & 71.1 (0.0) \\
& Gen: drop newline & 53.5 (-5.0) & 75.5 (+0.5) & 80.0 (+3.0) & 71.5 (-2.5) & 70.1 (-1.0) \\
& Gen: drop prompt, keep newline & 0.0 (-58.5) & 0.0 (-75.0) & 0.0 (-77.0) & 0.0 (-74.0) & 0.0 (-71.1) \\
& Gen: no image & 1.0 (-57.5) & 16.0 (-59.0) & 44.0 (-33.0) & 32.5 (-41.5) & 23.4 (-47.8) \\
& Gen: no text & 0.0 (-58.5) & 0.0 (-75.0) & 0.0 (-77.0) & 0.0 (-74.0) & 0.0 (-71.1) \\
& Prefill: no image & 0.0 (-58.5) & 0.0 (-75.0) & 0.0 (-77.0) & 0.0 (-74.0) & 0.0 (-71.1) \\
& Prefill no image + Gen no image & 0.0 (-58.5) & 0.0 (-75.0) & 0.0 (-77.0) & 0.0 (-74.0) & 0.0 (-71.1) \\
& Prefill no image + Gen no text & 0.0 (-58.5) & 0.0 (-75.0) & 0.0 (-77.0) & 0.0 (-74.0) & 0.0 (-71.1) \\
\bottomrule
\end{tabular}
\caption{All-layer attention knockout results across LIBERO suites. Each cell reports success rate (\%) and the absolute change relative to the suite-specific all-layer baseline in parentheses. The table uses the primary all-layer result directories rather than the auxiliary layer-wise scan directories. When duplicate runs exist within the same primary all-layer source, the success rate is averaged and the delta is recomputed from the intervention-matched baseline. The Avg. column averages over all four suites for each setting.}
\label{tab:attention_knockout_all_layers_summary}
\end{table*}


==> tabs/cka_summary.tex <==
\begin{table*}[ht!]
\centering
\small
\setlength{\tabcolsep}{3.5pt}
\begin{tabular}{llccccc}
\toprule
Model & Stage & COCO & LIBERO-10 & LIBERO-goal & LIBERO-spatial & LIBERO-object \\
\midrule
\multirow{3}{*}{$\pifive$} 
& C0 & 0.249 / \textbf{0.375}@L13 & 0.684 / \textbf{0.861}@L12 & 0.301 / \textbf{0.507}@L12 & 0.490 / \textbf{0.687}@L14 & 0.672 / \textbf{0.773}@L14 \\
& C1 & 0.351 / \textbf{0.659}@L1 & 0.707 / \textbf{0.924}@L2 & 0.486 / \textbf{0.872}@L15 & 0.513 / \textbf{0.745}@L15 & 0.548 / \textbf{0.814}@L2 \\
& C2 & 0.388 / \textbf{0.664}@L2 & 0.535 / \textbf{0.758}@L2 & 0.486 / \textbf{0.789}@L2 & 0.576 / \textbf{0.833}@L18 & 0.693 / \textbf{0.946}@L1 \\
\midrule
\multirow{2}{*}{OpenVLA} 
& C1 & 0.044 / \textbf{0.501}@L32 & 0.486 / \textbf{0.890}@L32 & 0.042 / \textbf{0.478}@L32 & 0.215 / \textbf{0.727}@L32 & 0.194 / \textbf{0.650}@L32 \\
& C2 & 0.038 / \textbf{0.493}@L1 & 0.463 / \textbf{0.922}@L32 & 0.043 / \textbf{0.787}@L32 & 0.169 / \textbf{0.909}@L32 & 0.116 / \textbf{0.873}@L32 \\
\bottomrule
\end{tabular}
\caption{Layer-mean / peak cross-modal CKA across training stages. Peak layer is shown after @. The layer mean describes the overall thickness of alignment across depth, while the peak value and its layer identify where the strongest linear image--text coupling occurs.}
\label{tab:cka_summary}
\end{table*}

==> tabs/layerwise_knockout.tex <==
\begin{table*}[ht!]
\centering
\scriptsize
\setlength{\tabcolsep}{3.5pt}
\begin{tabular}{lllcccc}
\toprule
Model & Dataset & Layer-wise intervention & Mean SR & Worst layer & Worst SR & Worst drop \\
\midrule
$\pifive$ & LIBERO-10 & Prefill no V--L & 92.83 & L5 & 90.00 & -3.00 \\
$\pifive$ & LIBERO-10 & Generation no text & 92.67 & L11 & 91.00 & -2.00 \\
$\pifive$ & LIBERO-10 & Generation no image & 91.47 & L14 & 74.50 & -18.50 \\
$\pifive$ & LIBERO-10 & Prefill no V--L + generation no text & 92.89 & L7 & 89.50 & -3.50 \\
$\pifive$ & LIBERO-10 & Prefill no V--L + generation no image & 91.28 & L14 & 65.50 & -27.50 \\
\midrule
$\pifive$ & LIBERO-goal & Generation drop BOS+newline & 97.08 & L0 & 95.00 & -1.00 \\
$\pifive$ & LIBERO-goal & Generation drop instruction & 96.75 & L1 & 95.50 & -0.50 \\
$\pifive$ & LIBERO-goal & Generation keep BOS+newline only & 69.11 & L13 & 14.50 & -81.50 \\
$\pifive$ & LIBERO-goal & Generation no image & 79.92 & L13 & 34.50 & -61.50 \\
$\pifive$ & LIBERO-goal & Generation no text & 96.67 & L9 & 93.50 & -2.50 \\
$\pifive$ & LIBERO-goal & Prefill no V--L & 81.64 & L6 & 28.00 & -68.00 \\
$\pifive$ & LIBERO-goal & Prefill no V--L + generation no image & 60.64 & L11 & 21.50 & -74.50 \\
$\pifive$ & LIBERO-goal & Prefill no V--L + generation no text & 80.81 & L6 & 23.00 & -73.00 \\
\midrule
$\pifive$ & LIBERO-object & Generation drop BOS+newline & 98.86 & L9 & 97.50 & -1.00 \\
$\pifive$ & LIBERO-object & Generation drop instruction & 98.72 & L5 & 97.50 & -1.00 \\
$\pifive$ & LIBERO-object & Generation keep BOS+newline only & 72.89 & L11 & 10.50 & -88.00 \\
$\pifive$ & LIBERO-object & Generation no image & 85.25 & L11 & 43.00 & -55.50 \\
$\pifive$ & LIBERO-object & Generation no text & 98.78 & L1 & 97.50 & -1.00 \\
$\pifive$ & LIBERO-object & Prefill no V--L & 96.03 & L5 & 84.00 & -14.50 \\
$\pifive$ & LIBERO-object & Prefill no V--L + generation no image & 77.25 & L11 & 10.50 & -88.00 \\
$\pifive$ & LIBERO-object & Prefill no V--L + generation no text & 96.06 & L4 & 85.00 & -13.50 \\
\midrule
$\pifive$ & LIBERO-spatial & Generation drop BOS+newline & 99.08 & L5 & 97.50 & -1.00 \\
$\pifive$ & LIBERO-spatial & Generation drop instruction & 98.53 & L17 & 95.50 & -3.00 \\
$\pifive$ & LIBERO-spatial & Generation keep BOS+newline only & 70.58 & L13 & 7.50 & -91.00 \\
$\pifive$ & LIBERO-spatial & Generation no image & 79.14 & L13 & 33.00 & -65.50 \\
$\pifive$ & LIBERO-spatial & Generation no text & 98.64 & L0 & 96.50 & -2.00 \\
$\pifive$ & LIBERO-spatial & Prefill no V--L & 94.86 & L6 & 81.50 & -17.00 \\
$\pifive$ & LIBERO-spatial & Prefill no V--L + generation no image & 71.17 & L11 & 8.00 & -90.50 \\
$\pifive$ & LIBERO-spatial & Prefill no V--L + generation no text & 94.58 & L5 & 82.50 & -16.00 \\
\midrule
OpenVLA & LIBERO-10 & Generation drop newline & 52.88 & L5 & 44.50 & -13.50 \\
OpenVLA & LIBERO-10 & Generation drop prompt, keep newline & 51.80 & L15 & 38.50 & -19.50 \\
OpenVLA & LIBERO-10 & Generation no text & 50.89 & L15 & 35.00 & -23.00 \\
OpenVLA & LIBERO-10 & Generation no image & 53.16 & L10 & 45.50 & -12.50 \\
OpenVLA & LIBERO-10 & Prefill no image & 51.09 & L11 & 25.50 & -32.50 \\
OpenVLA & LIBERO-10 & Prefill no image + generation no text & 48.76 & L15 & 22.50 & -35.50 \\
\midrule
OpenVLA & LIBERO-goal & Generation drop newline & 75.58 & L13 & 70.00 & -9.50 \\
OpenVLA & LIBERO-goal & Generation drop prompt, keep newline & 45.75 & L2 & 0.00 & -79.50 \\
OpenVLA & LIBERO-goal & Generation no image & 67.72 & L12 & 49.00 & -30.50 \\
OpenVLA & LIBERO-goal & Generation no text & 42.69 & L2 & 0.00 & -79.50 \\
OpenVLA & LIBERO-goal & Prefill no image & 45.73 & L11 & 0.00 & -79.50 \\
OpenVLA & LIBERO-goal & Prefill no image + generation no image & 45.69 & L11 & 0.00 & -79.50 \\
OpenVLA & LIBERO-goal & Prefill no image + generation no text & 34.61 & L2 & 0.00 & -79.50 \\
\midrule
OpenVLA & LIBERO-object & Generation drop newline & 74.06 & L28 & 68.50 & -5.50 \\
OpenVLA & LIBERO-object & Generation drop prompt, keep newline & 49.98 & L2 & 0.00 & -74.00 \\
OpenVLA & LIBERO-object & Generation no image & 68.53 & L10 & 53.00 & -21.00 \\
OpenVLA & LIBERO-object & Generation no text & 47.33 & L2 & 0.00 & -74.00 \\
OpenVLA & LIBERO-object & Prefill no image & 43.44 & L2 & 0.00 & -74.00 \\
OpenVLA & LIBERO-object & Prefill no image + generation no image & 43.44 & L2 & 0.00 & -74.00 \\
OpenVLA & LIBERO-object & Prefill no image + generation no text & 33.66 & L1 & 0.00 & -74.00 \\
\midrule
OpenVLA & LIBERO-spatial & Generation drop newline & 78.28 & L6 & 74.50 & -2.50 \\
OpenVLA & LIBERO-spatial & Generation drop prompt, keep newline & 49.25 & L2 & 0.00 & -77.00 \\
OpenVLA & LIBERO-spatial & Generation no image & 74.09 & L13 & 63.00 & -14.00 \\
OpenVLA & LIBERO-spatial & Generation no text & 46.47 & L2 & 0.00 & -77.00 \\
OpenVLA & LIBERO-spatial & Prefill no image & 49.16 & L12 & 0.00 & -77.00 \\
OpenVLA & LIBERO-spatial & Prefill no image + generation no image & 49.89 & L3 & 0.50 & -76.50 \\
OpenVLA & LIBERO-spatial & Prefill no image + generation no text & 36.72 & L1 & 0.00 & -77.00 \\
\bottomrule
\end{tabular}
\caption{Unified layer-wise knockout summary across models and LIBERO suites. Mean SR averages success rates across scanned layers; Worst SR and Worst drop report the most damaging layer-wise intervention relative to the corresponding layer-wise baseline. The $\pifive$ LIBERO-10 scan covers L0--L17; the OpenVLA LIBERO-10 scan covers L0--L31 except for one missing terminal-layer record in the combined prefill-image/generation-text setting.}
\label{tab:layerwise_knockout_summary}
\end{table*}

==> tabs/patch_mask_1.tex <==
\begin{table*}[t]
\centering
\scriptsize
\begin{tabular}{llccccccccccc}
\toprule
Model & Setting & Avg & t0 & t1 & t2 & t3 & t4 & t5 & t6 & t7 & t8 & t9 \\
\midrule

\multirow{15}{*}{$\pifive$}
& Baseline & 75.00 & 56.00 & 98.00 & 64.00 & 90.00 & 76.00 & 86.00 & 70.00 & 96.00 & 58.00 & 56.00 \\
\cmidrule{2-13}
& Target (BG) & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
& Target (Black) & 19.60 & 12.00 & 64.00 & 20.00 & 2.00 & 0.00 & 60.00 & 0.00 & 38.00 & 0.00 & 0.00 \\
& Target (Mosaic) & 47.20 & 82.00 & 96.00 & 34.00 & 8.00 & 22.00 & 94.00 & 22.00 & 58.00 & 54.00 & 2.00 \\
\cmidrule{2-13}
& Gripper (BG) & 8.40 & 6.00 & 0.00 & 0.00 & 4.00 & 18.00 & 54.00 & 0.00 & 2.00 & 0.00 & 0.00 \\
& Gripper (Black) & 52.60 & 60.00 & 96.00 & 6.00 & 60.00 & 46.00 & 68.00 & 52.00 & 78.00 & 24.00 & 36.00 \\
& Gripper (Mosaic) & 53.20 & 62.00 & 90.00 & 2.00 & 56.00 & 72.00 & 84.00 & 82.00 & 60.00 & 14.00 & 10.00 \\
\cmidrule{2-13}
& Robot (BG) & 3.40 & 0.00 & 0.00 & 0.00 & 2.00 & 12.00 & 20.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
& Robot (Black) & 30.20 & 50.00 & 90.00 & 0.00 & 32.00 & 8.00 & 34.00 & 34.00 & 34.00 & 0.00 & 20.00 \\
& Robot (Mosaic) & 39.20 & 54.00 & 64.00 & 0.00 & 32.00 & 64.00 & 38.00 & 72.00 & 66.00 & 2.00 & 0.00 \\
\cmidrule{2-13}
& Robot w/o Gripper (BG) & 52.60 & 70.00 & 96.00 & 0.00 & 36.00 & 66.00 & 44.00 & 44.00 & 94.00 & 44.00 & 32.00 \\
& Robot w/o Gripper (Black) & 58.40 & 80.00 & 94.00 & 0.00 & 84.00 & 58.00 & 58.00 & 52.00 & 90.00 & 26.00 & 42.00 \\
& Robot w/o Gripper (Mosaic) & 64.40 & 66.00 & 98.00 & 4.00 & 92.00 & 72.00 & 62.00 & 78.00 & 86.00 & 58.00 & 28.00 \\
\cmidrule{2-13}
& Background (Black) & 41.00 & 56.00 & 70.00 & 0.00 & 14.00 & 52.00 & 84.00 & 52.00 & 76.00 & 0.00 & 6.00 \\
& Background (Mosaic) & 57.80 & 60.00 & 98.00 & 8.00 & 94.00 & 56.00 & 88.00 & 54.00 & 44.00 & 42.00 & 34.00 \\
\midrule

\multirow{15}{*}{OpenVLA}
& Baseline & 54.33 & 50.00 & 83.33 & 56.67 & 36.67 & 50.00 & 70.00 & 36.67 & 76.67 & 43.33 & 40.00 \\
\cmidrule{2-13}
& Target (BG) & 5.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 50.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
& Target (Black) & 20.67 & 33.33 & 43.33 & 10.00 & 0.00 & 26.67 & 73.33 & 3.33 & 16.67 & 0.00 & 0.00 \\
& Target (Mosaic) & 25.00 & 16.67 & 60.00 & 6.67 & 3.33 & 16.67 & 76.67 & 10.00 & 50.00 & 6.67 & 3.33 \\
\cmidrule{2-13}
& Gripper (BG) & 10.67 & 10.00 & 6.67 & 23.33 & 10.00 & 10.00 & 3.33 & 40.00 & 3.33 & 0.00 & 0.00 \\
& Gripper (Black) & 31.33 & 23.33 & 46.67 & 36.67 & 16.67 & 30.00 & 36.67 & 30.00 & 53.33 & 3.33 & 36.67 \\
& Gripper (Mosaic) & 20.33 & 33.33 & 23.33 & 50.00 & 6.67 & 20.00 & 30.00 & 13.33 & 20.00 & 6.67 & 0.00 \\
\cmidrule{2-13}
& Robot (BG) & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
& Robot (Black) & 0.67 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 6.67 & 0.00 & 0.00 & 0.00 & 0.00 \\
& Robot (Mosaic) & 0.33 & 3.33 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
\cmidrule{2-13}
& Robot w/o Gripper (BG) & 10.00 & 10.00 & 13.33 & 0.00 & 0.00 & 26.67 & 43.33 & 6.67 & 0.00 & 0.00 & 0.00 \\
& Robot w/o Gripper (Black) & 11.67 & 13.33 & 16.67 & 0.00 & 0.00 & 23.33 & 46.67 & 3.33 & 10.00 & 3.33 & 0.00 \\
& Robot w/o Gripper (Mosaic) & 16.00 & 30.00 & 23.33 & 0.00 & 0.00 & 16.67 & 36.67 & 23.33 & 30.00 & 0.00 & 0.00 \\
\cmidrule{2-13}
& Background (Black) & 26.33 & 30.00 & 46.67 & 10.00 & 16.67 & 20.00 & 53.33 & 10.00 & 36.67 & 6.67 & 33.33 \\
& Background (Mosaic) & 48.00 & 46.67 & 73.33 & 30.00 & 36.67 & 56.67 & 76.67 & 56.67 & 53.33 & 20.00 & 30.00 \\

\bottomrule
\end{tabular}
\caption{Success rates (\%) across tasks and masking strategies on \textbf{LIBERO-10}. The instruction is provided in Table \ref{tab:patch_mask_1_ins}.} \label{tab:mask1}
\end{table*}


==> tabs/patch_mask_1_ins.tex <==
\begin{table}[ht!]
\begin{tcolorbox}[fontupper=\small, fontlower=\small]
t0: put both the alphabet soup and the tomato sauce in the basket.	\\
t1: put both the cream cheese box and the butter in the basket.	\\
t2: turn on the stove and put the moka pot on it.	\\
t3: put the black bowl in the bottom drawer of the cabinet and close it.\\	
t4: put the white mug on the left plate and put the yellow and white mug on the right plate.	\\
t5: pick up the book and place it in the back compartment of the caddy.	\\
t6: put the white mug on the plate and put the chocolate pudding to the right of the plate.	\\
t7: put both the alphabet soup and the cream cheese box in the basket.	\\
t8: put both moka pots on the stove.	\\
t9: put the yellow and white mug in the microwave and close it.	
\end{tcolorbox}
\caption{LIBERO-10: Instruction.}
\label{tab:patch_mask_1_ins}
\end{table}


==> tabs/patch_mask_1_oft.tex <==
\begin{table*}[t]
\centering
\scriptsize
\begin{tabular}{llccccccccccc}
\toprule
Model & Setting & Avg & t0 & t1 & t2 & t3 & t4 & t5 & t6 & t7 & t8 & t9 \\
\midrule

\multirow{15}{*}{OpenVLA-OFT}
& Baseline & 94.80 & 98.00 & 96.00 & 100.00 & 94.00 & 98.00 & 100.00 & 82.00 & 100.00 & 88.00 & 92.00 \\
\cmidrule{2-13}
& Target (BG) & 10.40 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 100.00 & 0.00 & 4.00 & 0.00 & 0.00\\
& Target (Black) & 15.20 & 10.00 & 16.00 & 2.00 & 0.00 & 0.00 & 100.00 & 0.00 & 24.00 & 0.00 & 0.00 \\
& Target (Mosaic) & 48.20 & 86.00 & 98.00 & 0.00 & 78.00 & 14.00 & 100.00 & 4.00 & 96.00 & 0.00 & 6.00 \\
\cmidrule{2-13}
& Gripper (BG) & 89.80 & 92.00 & 100.00 & 92.00 & 94.00 & 100.00 & 98.00 & 86.00 & 86.00 & 64.00 & 86.00 \\
& Gripper (Black) & 89.80 & 92.00 & 98.00 & 98.00 & 90.00 & 96.00 & 94.00 & 84.00 & 98.00 & 60.00 & 88.00 \\
& Gripper (Mosaic) & 95.00 & 98.00 & 94.00 & 92.00 & 98.00 & 98.00 & 96.00 & 92.00 & 98.00 & 88.00 & 96.00 \\
\cmidrule{2-13}
& Robot (BG) & 66.80 & 68.00 & 66.00 & 54.00 & 82.00 & 88.00 & 80.00 & 50.00 & 88.00 & 30.00 & 62.00 \\
& Robot (Black) & 79.00 & 86.00 & 92.00 & 66.00 & 86.00 & 96.00 & 84.00 & 52.00 & 94.00 & 52.00 & 82.00 \\
& Robot (Mosaic) & 84.40 & 90.00 & 96.00 & 70.00 & 100.00 & 92.00 & 88.00 & 92.00 & 98.00 & 30.00 & 88.00 \\
\cmidrule{2-13}
& Robot w/o Gripper (BG) & 85.40 & 88.00 & 88.00 & 94.00 & 90.00 & 96.00 & 98.00 & 54.00 & 100.00 & 58.00 & 88.00 \\
& Robot w/o Gripper (Black) & 84.00 & 92.00 & 94.00 & 96.00 & 84.00 & 98.00 & 96.00 & 46.00 & 98.00 & 56.00 & 80.00 \\
& Robot w/o Gripper (Mosaic) & 91.20 & 92.00 & 96.00 & 94.00 & 100.00 & 98.00 & 98.00 & 94.00 & 98.00 & 50.00 & 92.00 \\
\cmidrule{2-13}
& Background (Black) & 73.80 & 100.00 & 92.00 & 86.00 & 90.00 & 92.00 & 84.00 & 62.00 & 96.00 & 8.00 & 28.00 \\
& Background (Mosaic) & 84.60 & 92.00 & 98.00 & 80.00 & 92.00 & 84.00 & 100.00 & 76.00 & 100.00 & 40.00 & 84.00 \\

\bottomrule
\end{tabular}
\caption{Success rates (\%) across tasks and masking strategies on \textbf{LIBERO-10} for OpenVLA-OFT. The instruction is provided in Table \ref{tab:patch_mask_1_ins}.} \label{tab:mask1_oft}
\end{table*}


==> tabs/patch_mask_2.tex <==
\begin{table*}[t]
\centering
\scriptsize
\begin{tabular}{llccccccccccc}
\toprule
Model & Setting & Avg & t0 & t1 & t2 & t3 & t4 & t5 & t6 & t7 & t8 & t9 \\
\midrule

\multirow{15}{*}{$\pifive$}
& Baseline & 95.60 & 96.00 & 98.00 & 78.00 & 98.00 & 90.00 & 100.00 & 100.00 & 96.00 & 100.00 & 100.00  \\
\cmidrule{2-13}
& Target (BG) & 13.00 & 8.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 52.00 & 0.00 & 70.00 & 0.00\\
& Target (Black) & 61.60 & 16.00 & 94.00 & 44.00 & 94.00 & 94.00 & 24.00 & 72.00 & 90.00 & 88.00 & 0.00 \\
& Target (Mosaic) & 74.00 & 58.00 & 94.00 & 22.00 & 86.00 & 96.00 & 14.00 & 90.00 & 90.00 & 92.00 & 98.00 \\
\cmidrule{2-13}
& Gripper (BG) & 3.20 & 2.00 & 2.00 & 0.00 & 0.00 & 24.00 & 0.00 & 0.00 & 0.00 & 4.00 & 0.00 \\
& Gripper (Black) & 97.40 & 100.00 & 100.00 & 86.00 & 96.00 & 100.00 & 98.00 & 98.00 & 96.00 & 100.00 & 100.00 \\
& Gripper (Mosaic) & 79.40 & 100.00 & 96.00 & 24.00 & 76.00 & 100.00 & 26.00 & 100.00 & 100.00 & 98.00 & 74.00 \\
\cmidrule{2-13}
& Robot (BG) & 26.40 & 8.00 & 52.00 & 8.00 & 24.00 & 64.00 & 0.00 & 10.00 & 58.00 & 40.00 & 0.00 \\
& Robot (Black)& 93.60 & 94.00 & 98.00 & 90.00 & 84.00 & 92.00 & 98.00 & 90.00 & 100.00 & 96.00 & 94.00 \\
& Robot (Mosaic) & 74.60 & 100.00 & 96.00 & 26.00 & 76.00 & 100.00 & 20.00 & 100.00 & 100.00 & 94.00 & 34.00 \\
\cmidrule{2-13}
& Robot w/o Gripper (BG) & 91.80 & 94.00 & 98.00 & 90.00 & 76.00 & 66.00 & 98.00 & 100.00 & 96.00 & 100.00 & 100.00 \\
& Robot w/o Gripper (Black) & 92.80 & 94.00 & 100.00 & 90.00 & 88.00 & 66.00 & 98.00 & 96.00 & 100.00 & 100.00 & 96.00 \\
& Robot w/o Gripper (Mosaic) & 96.60 & 100.00 & 98.00 & 80.00 & 98.00 & 96.00 & 100.00 & 98.00 & 98.00 & 100.00 & 98.00 \\
\cmidrule{2-13}
& Background (Black) & 79.40&	66.00&	100.00&	80.00&	78.00&	100.00&	68.00&	62.00&	68.00&	88.00&	84.00 \\
& Background (Mosaic) & 86.60&	96.00&	96.00&	22.00&	78.00&	100.00&	88.00&	92.00&	98.00&	100.00&	96.00 \\
\midrule

\multirow{15}{*}{OpenVLA}
& Baseline & 70.00 & 63.33 & 76.67 & 70.00 & 46.67 & 83.33 & 73.33 & 63.33 & 76.67 & 60.00 & 86.67 \\
\cmidrule{2-13}
& Target (BG) & 0.33 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 3.33 & 0.00 & 0.00 & 0.00 \\
& Target (Black) & 55.67 & 83.33 & 46.67 & 73.33 & 43.33 & 63.33 & 80.00 & 50.00 & 73.33 & 20.00 & 23.33 \\
& Target (Mosaic) & 59.67 & 70.00 & 50.00 & 56.67 & 26.67 & 76.67 & 63.33 & 63.33 & 86.67 & 60.00 & 43.33 \\
\cmidrule{2-13}
& Gripper (BG) & 1.00 & 0.00 & 0.00 & 6.67 & 3.33 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
& Gripper (Black) & 72.00 & 73.33 & 40.00 & 80.00 & 56.67 & 80.00 & 80.00 & 86.67 & 96.67 & 43.33 & 83.33 \\
& Gripper (Mosaic) & 3.67 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 36.67 \\
\cmidrule{2-13}
& Robot (BG) & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
& Robot (Black) & 4.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 36.67 & 0.00 & 0.00 & 0.00 & 3.33 \\
& Robot (Mosaic) & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
\cmidrule{2-13}
& Robot w/o Gripper (BG) & 34.33 & 73.33 & 33.33 & 43.33 & 56.67 & 33.33 & 6.67 & 0.00 & 6.67 & 10.00 & 80.00 \\
& Robot w/o Gripper (Black) & 17.33 & 0.00 & 16.67 & 36.67 & 26.67 & 0.00 & 23.33 & 0.00 & 0.00 & 0.00 & 70.00 \\
& Robot w/o Gripper (Mosaic) & 15.67 & 50.00 & 13.33 & 10.00 & 30.00 & 3.33 & 6.67 & 0.00 & 6.67 & 0.00 & 36.67 \\
\cmidrule{2-13}
& Background (Black) & 42.67 & 63.33 & 23.33 & 43.33 & 40.00 & 66.67 & 0.00 & 6.67 & 73.33 & 50.00 & 60.00 \\
& Background (Mosaic) & 65.67 & 76.67 & 56.67 & 83.33 & 53.33 & 93.33 & 63.33 & 40.00 & 76.67 & 40.00 & 73.33 \\

\bottomrule
\end{tabular}
\caption{Success rates comparison across tasks and masking strategies on \textbf{LIBERO-Object}. The instruction is provided in Table \ref{tab:patch_mask_2_ins}.} \label{tab:mask2}
\end{table*}							

==> tabs/patch_mask_2_ins.tex <==
\begin{table}[t]
\begin{tcolorbox}[fontupper=\small, fontlower=\small]
t0: pick up the alphabet soup and place it in the basket \\
t1: pick up the cream cheese and place it in the basket \\
t2: pick up the salad dressing and place it in the basket \\
t3: pick up the bbq sauce and place it in the basket \\
t4: pick up the ketchup and place it in the basket \\
t5: pick up the tomato sauce and place it in the basket \\
t6: pick up the butter and place it in the basket \\
t7: pick up the milk and place it in the basket \\
t8: pick up the chocolate pudding and place it in the basket \\
t9: pick up the orange juice and place it in the basket									
\end{tcolorbox}
\caption{LIBERO-Object: Instruction}
\label{tab:patch_mask_2_ins}
\end{table}

==> tabs/patch_mask_2_oft.tex <==
\begin{table*}[t]
\centering
\scriptsize
\begin{tabular}{llccccccccccc}
\toprule
Model & Setting & Avg & t0 & t1 & t2 & t3 & t4 & t5 & t6 & t7 & t8 & t9 \\
\midrule

\multirow{15}{*}{OpenVLA-OFT}
& Baseline & 99.80 & 100.00 & 100.00 & 98.00 & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 \\
\cmidrule{2-13}
& Target (BG) & 57.00 & 94.00 & 0.00 & 16.00 & 46.00 & 38.00 & 80.00 & 94.00 & 12.00 & 96.00 & 94.00 \\
& Target (Black) & 84.80 & 70.00 & 32.00 & 100.00 & 96.00 & 100.00 & 100.00 & 98.00 & 80.00 & 74.00 & 98.00 \\
& Target (Mosaic) & 98.40 & 94.00 & 96.00 & 98.00 & 98.00 & 100.00 & 98.00 & 100.00 & 100.00 & 100.00 & 100.00 \\
\cmidrule{2-13}
& Gripper (BG) & 94.20 & 100.00 & 100.00 & 100.00 & 94.00 & 66.00 & 100.00 & 96.00 & 88.00 & 100.00 & 98.00 \\
& Gripper (Black) & 98.80 & 96.00 & 100.00 & 100.00 & 98.00 & 100.00 & 100.00 & 96.00 & 100.00 & 98.00 & 100.00 \\
& Gripper (Mosaic) & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 \\
\cmidrule{2-13}
& Robot (BG) & 96.00 & 98.00 & 100.00 & 100.00 & 98.00 & 92.00 & 100.00 & 92.00 & 86.00 & 96.00 & 98.00 \\
& Robot (Black) & 96.80 & 98.00 & 98.00 & 96.00 & 98.00 & 96.00 & 98.00 & 92.00 & 96.00 & 100.00 & 96.00 \\
& Robot (Mosaic) & 97.60 & 100.00 & 92.00 & 100.00 & 98.00 & 96.00 & 100.00 & 96.00 & 96.00 & 98.00 & 100.00 \\
\cmidrule{2-13}
& Robot w/o Gripper (BG) & 98.60 & 100.00 & 100.00 & 98.00 & 100.00 & 100.00 & 98.00 & 98.00 & 100.00 & 100.00 & 92.00 \\
& Robot w/o Gripper (Black) & 99.80 & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 98.00 & 100.00 & 100.00 & 100.00 \\
& Robot w/o Gripper (Mosaic) & 98.80 & 100.00 & 98.00 & 100.00 & 96.00 & 100.00 & 98.00 & 98.00 & 100.00 & 100.00 & 98.00 \\
\cmidrule{2-13}
& Background (Black) & 47.40 & 96.00 & 2.00 & 2.00 & 16.00 & 86.00 & 52.00 & 70.00 & 24.00 & 100.00 & 26.00 \\
& Background (Mosaic) & 95.00 & 100.00 & 86.00 & 98.00 & 100.00 & 96.00 & 88.00 & 94.00 & 98.00 & 100.00 & 90.00 \\

\bottomrule
\end{tabular}
\caption{Success rates (\%) across tasks and masking strategies on \textbf{LIBERO-Object} for OpenVLA-OFT. The instruction is provided in Table \ref{tab:patch_mask_2_ins}.} \label{tab:mask2_oft}
\end{table*}


==> tabs/patch_mask_3.tex <==
\begin{table*}[t]
\centering
\scriptsize
\begin{tabular}{llccccccccccc}
\toprule
Model & Setting & Avg & t0 & t1 & t2 & t3 & t4 & t5 & t6 & t7 & t8 & t9 \\
\midrule

\multirow{15}{*}{$\pifive$}
& Baseline & 95.80 & 100.00 & 92.00 & 100.00 & 100.00 & 88.00 & 100.00 & 100.00 & 96.00 & 86.00 & 96.00 \\
\cmidrule{2-13}
& Target (BG) & 7.80 & 0.00 & 0.00 & 0.00 & 0.00 & 8.00 & 0.00 & 0.00 & 52.00 & 0.00 & 18.00 \\
& Target (Black) & 23.00 & 44.00 & 12.00 & 64.00 & 6.00 & 0.00 & 2.00 & 24.00 & 64.00 & 0.00 & 14.00 \\
& Target (Mosaic) & 50.20 & 74.00 & 64.00 & 46.00 & 62.00 & 20.00 & 16.00 & 78.00 & 76.00 & 20.00 & 46.00 \\
\cmidrule{2-13}
& Gripper (BG) & 64.00 & 76.00 & 66.00 & 100.00 & 64.00 & 20.00 & 72.00 & 84.00 & 98.00 & 60.00 & 0.00 \\
& Gripper (Black) & 94.80 & 100.00 & 94.00 & 100.00 & 96.00 & 78.00 & 98.00 & 100.00 & 100.00 & 90.00 & 92.00\\
& Gripper (Mosaic) & 89.80 & 100.00 & 94.00 & 100.00 & 92.00 & 58.00 & 94.00 & 100.00 & 98.00 & 90.00 & 72.00 \\
\cmidrule{2-13}
& Robot (BG) & 47.60 & 78.00 & 2.00 & 92.00 & 44.00 & 4.00 & 68.00 & 94.00 & 86.00 & 8.00 & 0.00 \\
& Robot (Black)& 95.00 & 100.00 & 98.00 & 98.00 & 94.00 & 84.00 & 98.00 & 100.00 & 96.00 & 94.00 & 88.00 \\
& Robot (Mosaic) & 89.60 & 100.00 & 98.00 & 100.00 & 82.00 & 66.00 & 94.00 & 98.00 & 100.00 & 88.00 & 70.00 \\
\cmidrule{2-13}
& Robot w/o Gripper (BG) & 97.40 & 98.00 & 100.00 & 98.00 & 100.00 & 92.00 & 96.00 & 100.00 & 100.00 & 92.00 & 98.00 \\
& Robot w/o Gripper (Black) & 99.00 & 98.00 & 98.00 & 100.00 & 100.00 & 98.00 & 100.00 & 100.00 & 100.00 & 96.00 & 100.00 \\
& Robot w/o Gripper (Mosaic) & 96.40 & 100.00 & 96.00 & 96.00 & 100.00 & 92.00 & 96.00 & 100.00 & 94.00 & 92.00 & 98.00 \\
\cmidrule{2-13}
& Background (Black) & 67.20&	96.00&	46.00&	94.00&	58.00&	54.00&	30.00&	100.00&	92.00&	26.00&	76.00 \\
& Background (Mosaic) & 93.00&	100.00&	96.00&	100.00&	96.00&	68.00&	100.00&	98.00&	94.00&	84.00&	94.00 \\
\midrule

\multirow{15}{*}{OpenVLA}
& Baseline & 79.67 & 86.67 & 90.00 & 80.00 & 100.00 & 76.67 & 46.67 & 86.67 & 76.67 & 83.33 & 70.00 \\
\cmidrule{2-13}
& Target (BG) & 36.67 & 26.67 & 83.33 & 43.33 & 36.67 & 3.33 & 0.00 & 66.67 & 70.00 & 16.67 & 20.00 \\
& Target (Black) & 63.33 & 60.00 & 93.33 & 63.33 & 86.67 & 63.33 & 3.33 & 80.00 & 90.00 & 50.00 & 43.33 \\
& Target (Mosaic) & 70.00 & 83.33 & 93.33 & 76.67 & 83.33 & 60.00 & 30.00 & 86.67 & 80.00 & 63.33 & 43.33 \\
\cmidrule{2-13}
& Gripper (BG) & 19.00 & 23.33 & 0.00 & 10.00 & 26.67 & 13.33 & 0.00 & 23.33 & 40.00 & 53.33 & 0.00 \\
& Gripper (Black) & 70.67 & 80.00 & 70.00 & 93.33 & 86.67 & 56.67 & 13.33 & 90.00 & 80.00 & 73.33 & 63.33 \\
& Gripper (Mosaic) & 53.00 & 56.67 & 73.33 & 46.67 & 90.00 & 6.67 & 0.00 & 73.33 & 60.00 & 76.67 & 46.67 \\
\cmidrule{2-13}
& Robot (BG) & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
& Robot (Black) & 3.33 & 0.00 & 13.33 & 0.00 & 0.00 & 3.33 & 0.00 & 0.00 & 0.00 & 16.67 & 0.00 \\
& Robot (Mosaic) & 2.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 16.67 & 3.33 \\
\cmidrule{2-13}
& Robot w/o Gripper (BG) & 22.00 & 13.33 & 16.67 & 46.67 & 43.33 & 26.67 & 0.00 & 10.00 & 0.00 & 23.33 & 40.00 \\
& Robot w/o Gripper (Black) & 31.67 & 46.67 & 46.67 & 33.33 & 70.00 & 46.67 & 0.00 & 33.33 & 6.67 & 23.33 & 10.00 \\
& Robot w/o Gripper (Mosaic) & 49.67 & 43.33 & 76.67 & 73.33 & 60.00 & 66.67 & 0.00 & 33.33 & 43.33 & 63.33 & 36.67 \\
\cmidrule{2-13}
& Background (Black) & 47.33 & 43.33 & 3.33 & 46.67 & 100.00 & 56.67 & 3.33 & 83.33 & 23.33 & 70.00 & 43.33 \\
& Background (Mosaic) & 82.33 & 96.67 & 96.67 & 80.00 & 86.67 & 66.67 & 46.67 & 93.33 & 90.00 & 90.00 & 76.67 \\

\bottomrule
\end{tabular}
\caption{Success rates comparison across tasks and masking strategies on \textbf{LIBERO-Spatial}. The instruction is provided in Table \ref{tab:patch_mask_3_ins}.} \label{tab:mask3}
\end{table*}																																												

==> tabs/patch_mask_3_ins.tex <==
\begin{table}[t]
\begin{tcolorbox}[fontupper=\small, fontlower=\small]
t0: pick up the black bowl between the plate and the ramekin and place it on the plate \\
t1: pick up the black bowl next to the ramekin and place it on the plate \\
t2: pick up the black bowl from table center and place it on the plate \\
t3: pick up the black bowl on the cookie box and place it on the plate \\
t4: pick up the black bowl in the top drawer of the wooden cabinet and place it on the plate \\
t5: pick up the black bowl on the ramekin and place it on the plate \\
t6: pick up the black bowl next to the cookie box and place it on the plate \\
t7: pick up the black bowl on the stove and place it on the plate\\
t8: pick up the black bowl next to the plate and place it on the plate \\
t9: pick up the black bowl on the wooden cabinet and place it on the plate
\end{tcolorbox}
\caption{LIBERO-Spatial: Instruction.}
\label{tab:patch_mask_3_ins}
\end{table}

==> tabs/patch_mask_3_oft.tex <==
\begin{table*}[t]
\centering
\scriptsize
\begin{tabular}{llccccccccccc}
\toprule
Model & Setting & Avg & t0 & t1 & t2 & t3 & t4 & t5 & t6 & t7 & t8 & t9 \\
\midrule

\multirow{15}{*}{OpenVLA-OFT}
& Baseline & 92.80 & 100.00 & 98.00 & 100.00 & 100.00 & 96.00 & 46.00 & 100.00 & 94.00 & 96.00 & 98.00 \\
\cmidrule{2-13}
& Target (BG) & 26.80 & 26.00 & 0.00 & 10.00 & 26.00 & 56.00 & 0.00 & 30.00 & 18.00 & 10.00 & 92.00 \\
& Target (Black) & 35.40 & 14.00 & 54.00 & 0.00 & 58.00 & 42.00 & 2.00 & 44.00 & 18.00 & 32.00 & 90.00 \\
& Target (Mosaic) & 76.00 & 92.00 & 90.00 & 92.00 & 84.00 & 90.00 & 6.00 & 96.00 & 38.00 & 76.00 & 96.00 \\
\cmidrule{2-13}
& Gripper (BG) & 92.40 & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 36.00 & 98.00 & 96.00 & 96.00 & 98.00 \\
& Gripper (Black) & 92.80 & 100.00 & 100.00 & 98.00 & 100.00 & 100.00 & 46.00 & 98.00 & 96.00 & 94.00 & 96.00 \\
& Gripper (Mosaic) & 93.80 & 100.00 & 98.00 & 100.00 & 100.00 & 98.00 & 54.00 & 100.00 & 92.00 & 96.00 & 100.00 \\
\cmidrule{2-13}
& Robot (BG) & 81.40 & 86.00 & 84.00 & 100.00 & 94.00 & 88.00 & 30.00 & 82.00 & 90.00 & 66.00 & 94.00 \\
& Robot (Black) & 86.80 & 88.00 & 94.00 & 98.00 & 98.00 & 98.00 & 30.00 & 100.00 & 94.00 & 74.00 & 94.00 \\
& Robot (Mosaic) & 91.60 & 98.00 & 100.00 & 100.00 & 100.00 & 90.00 & 38.00 & 100.00 & 94.00 & 96.00 & 100.00 \\
\cmidrule{2-13}
& Robot w/o Gripper (BG) & 90.40 & 90.00 & 100.00 & 100.00 & 96.00 & 94.00 & 48.00 & 100.00 & 92.00 & 90.00 & 94.00 \\
& Robot w/o Gripper (Black) & 91.00 & 96.00 & 100.00 & 100.00 & 100.00 & 98.00 & 40.00 & 100.00 & 92.00 & 90.00 & 94.00 \\
& Robot w/o Gripper (Mosaic) & 91.20 & 98.00 & 100.00 & 96.00 & 100.00 & 98.00 & 34.00 & 100.00 & 96.00 & 94.00 & 96.00 \\
\cmidrule{2-13}
& Background (Black) & 83.20 & 96.00 & 88.00 & 100.00 & 100.00 & 82.00 & 0.00 & 100.00 & 94.00 & 86.00 & 86.00 \\
& Background (Mosaic) & 88.20 & 100.00 & 86.00 & 100.00 & 98.00 & 92.00 & 24.00 & 100.00 & 94.00 & 94.00 & 94.00 \\

\bottomrule
\end{tabular}
\caption{Success rates (\%) across tasks and masking strategies on \textbf{LIBERO-Spatial} for OpenVLA-OFT. The instruction is provided in Table \ref{tab:patch_mask_3_ins}.} \label{tab:mask3_oft}
\end{table*}


==> tabs/patch_mask_4_ins.tex <==
\begin{table}[t]
\begin{tcolorbox}[fontupper=\small, fontlower=\small]
t0: put carrot on plate \\
t1: put eggplant into yellow basket \\
t2: put the spoon on the towel \\
t3: stack the green block on the yellow block							
\end{tcolorbox}
\caption{Simpler: Instruction.}
\label{tab:patch_mask_4_ins}
\end{table}

==> tabs/patch_mask_goal.tex <==
\begin{table*}[htbp]
\centering
\scriptsize
\begin{tabular}{llccccccccccc}
\toprule
Model & Setting & Avg & t0 & t1 & t2 & t3 & t4 & t5 & t6 & t7 & t8 & t9 \\
\midrule

\multirow{15}{*}{$\pifive$}
& Baseline & 80.00 & 8.00 & 100.00 & 94.00 & 46.00 & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 52.00 \\
\cmidrule{2-13}
& Target(BG) & 19.80 & 6.00 & 12.00 & 52.00 & 2.00 & 10.00 & 6.00 & 14.00 & 68.00 & 20.00 & 8.00 \\
& Target(Black) & 58.80 & 4.00 & 70.00 & 92.00 & 2.00 & 76.00 & 54.00 & 54.00 & 100.00 & 56.00 & 80.00 \\
& Target(Mosaic) & 58.40 & 6.00 & 32.00 & 92.00 & 8.00 & 12.00 & 98.00 & 92.00 & 100.00 & 94.00 & 50.00 \\
\cmidrule{2-13}
& Gripper(BG) & 59.20 & 0.00 & 96.00 & 68.00 & 6.00 & 96.00 & 44.00 & 90.00 & 100.00 & 88.00 & 4.00 \\
& Gripper(Black) & 74.80 & 0.00 & 100.00 & 90.00 & 28.00 & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 30.00 \\
& Gripper(Mosaic) & 74.20 & 2.00 & 100.00 & 92.00 & 16.00 & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 32.00 \\
\cmidrule{2-13}
& Robot(BG) & 44.00 & 0.00 & 92.00 & 10.00 & 0.00 & 94.00 & 34.00 & 58.00 & 52.00 & 100.00 & 0.00 \\
& Robot(Black) & 69.80 & 6.00 & 100.00 & 78.00 & 18.00 & 100.00 & 98.00 & 98.00 & 100.00 & 100.00 & 0.00 \\
& Robot(Mosaic) & 68.60 & 6.00 & 100.00 & 40.00 & 18.00 & 100.00 & 92.00 & 98.00 & 100.00 & 100.00 & 32.00 \\
\cmidrule{2-13}
& Robot w/o Gripper(BG) & 76.80 & 2.00 & 100.00 & 76.00 & 46.00 & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 44.00 \\
& Robot w/o Gripper(Black) & 76.40 & 8.00 & 100.00 & 90.00 & 32.00 & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 34.00 \\
& Robot w/o Gripper(Mosaic) & 79.00 & 18.00 & 100.00 & 76.00 & 44.00 & 100.00 & 100.00 & 96.00 & 100.00 & 100.00 & 56.00 \\
\cmidrule{2-13}
& Background(Black) & 57.80 & 16.00 & 100.00 & 20.00 & 16.00 & 100.00 & 40.00 & 58.00 & 100.00 & 100.00 & 28.00 \\
& Background(Mosaic) & 78.00 & 2.00 & 100.00 & 90.00 & 36.00 & 100.00 & 100.00 & 96.00 & 100.00 & 100.00 & 56.00 \\
\midrule

\multirow{15}{*}{OpenVLA}
& Baseline & 74.00 & 53.33 & 93.33 & 80.00 & 43.33 & 93.33 & 80.00 & 63.33 & 93.33 & 83.33 & 56.67 \\
\cmidrule{2-13}
& Target(BG) & 45.00 & 53.33 & 60.00 & 30.00 & 46.67 & 73.33 & 73.33 & 3.33 & 46.67 & 26.67 & 36.67 \\
& Target(Black) & 73.00 & 73.33 & 83.33 & 83.33 & 46.67 & 83.33 & 73.33 & 50.00 & 93.33 & 76.67 & 66.67 \\
& Target(Mosaic) & 67.67 & 50.00 & 80.00 & 73.33 & 63.33 & 80.00 & 76.67 & 43.33 & 100.00 & 66.67 & 43.33 \\
\cmidrule{2-13}
& Gripper(BG) & 38.00 & 33.33 & 26.67 & 33.33 & 3.33 & 86.67 & 63.33 & 50.00 & 20.00 & 43.33 & 20.00 \\
& Gripper(Black) & 69.33 & 50.00 & 73.33 & 83.33 & 13.33 & 90.00 & 73.33 & 80.00 & 86.67 & 86.67 & 56.67 \\
& Gripper(Mosaic) & 63.00 & 20.00 & 60.00 & 63.33 & 30.00 & 100.00 & 70.00 & 80.00 & 96.67 & 63.33 & 46.67 \\
\cmidrule{2-13}
& Robot(BG) & 0.33 & 0.00 & 3.33 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
& Robot(Black) & 6.00 & 0.00 & 3.33 & 0.00 & 0.00 & 3.33 & 0.00 & 16.67 & 36.67 & 0.00 & 0.00 \\
& Robot(Mosaic) & 8.00 & 0.00 & 0.00 & 3.33 & 0.00 & 40.00 & 10.00 & 6.67 & 20.00 & 0.00 & 0.00 \\
\cmidrule{2-13}
& Robot w/o Gripper(BG) & 25.67 & 10.00 & 63.33 & 13.33 & 0.00 & 50.00 & 0.00 & 23.33 & 66.67 & 30.00 & 0.00 \\
& Robot w/o Gripper(Black) & 26.00 & 13.33 & 70.00 & 30.00 & 0.00 & 26.67 & 10.00 & 16.67 & 76.67 & 16.67 & 0.00 \\
& Robot w/o Gripper(Mosaic) & 38.33 & 6.67 & 70.00 & 53.33 & 10.00 & 80.00 & 30.00 & 13.33 & 66.67 & 53.33 & 0.00 \\
\cmidrule{2-13}
& Background(Black) & 41.67 & 33.33 & 56.67 & 3.33 & 13.33 & 63.33 & 86.67 & 43.33 & 80.00 & 26.67 & 10.00 \\
& Background(Mosaic) & 70.67 & 56.67 & 100.00 & 63.33 & 30.00 & 96.67 & 86.67 & 50.00 & 96.67 & 76.67 & 50.00 \\

\bottomrule
\end{tabular}
\caption{Success rates comparison across tasks and masking strategies on \textbf{LIBERO-Goal}. The instruction is provided in Table \ref{tab:patch_mask_goal_ins}.} \label{tab:mask_goal}
\end{table*}

==> tabs/patch_mask_goal_ins.tex <==
\begin{table}[t]
\begin{tcolorbox}[fontupper=\small, fontlower=\small]			
t0: open the middle drawer of the cabinet \\
t1: put the bowl on the stove	 \\
t2: put the wine bottle on top of the cabinet	 \\
t3: open the top drawer and put the bowl inside	 \\
t4: put the bowl on top of the cabinet	 \\
t5: push the plate to the front of the stove	 \\
t6: put the cream cheese in the bowl	 \\
t7: turn on the stove	 \\
t8: put the bowl on the plate	 \\
t9: put the wine bottle on the rack		 \\																					
\end{tcolorbox}
\caption{LIBERO-Goal: Instruction.}
\label{tab:patch_mask_goal_ins}
\end{table}

==> tabs/patch_mask_goal_oft.tex <==
\begin{table*}[t]
\centering
\scriptsize
\begin{tabular}{llccccccccccc}
\toprule
Model & Setting & Avg & t0 & t1 & t2 & t3 & t4 & t5 & t6 & t7 & t8 & t9 \\
\midrule

\multirow{15}{*}{OpenVLA-OFT}
& Baseline & 97.40 & 98.00 & 100.00 & 94.00 & 96.00 & 100.00 & 96.00 & 94.00 & 100.00 & 100.00 & 96.00 \\
\cmidrule{2-13}
& Target (BG) & 49.60 & 98.00 & 82.00 & 68.00 & 38.00 & 72.00 & 0.00 & 4.00 & 34.00 & 18.00 & 82.00 \\
& Target (Black) & 60.20 & 98.00 & 90.00 & 94.00 & 46.00 & 86.00 & 0.00 & 2.00 & 86.00 & 0.00 & 100.00 \\
& Target (Mosaic) & 88.40 & 98.00 & 96.00 & 96.00 & 82.00 & 98.00 & 68.00 & 74.00 & 78.00 & 96.00 & 98.00 \\
\cmidrule{2-13}
& Gripper (BG) & 96.00 & \multicolumn{10}{c}{--} \\
& Gripper (Black) & 97.00 & 98.00 & 98.00 & 98.00 & 90.00 & 98.00 & 100.00 & 96.00 & 98.00 & 96.00 & 98.00 \\
& Gripper (Mosaic) & 97.60 & 98.00 & 100.00 & 98.00 & 90.00 & 100.00 & 98.00 & 94.00 & 100.00 & 100.00 & 98.00 \\
\cmidrule{2-13}
& Robot (BG) & 67.20 & 94.00 & 50.00 & 96.00 & 16.00 & 100.00 & 70.00 & 60.00 & 18.00 & 92.00 & 76.00 \\
& Robot (Black) & 87.20 & 100.00 & 76.00 & 92.00 & 62.00 & 98.00 & 96.00 & 70.00 & 96.00 & 96.00 & 86.00 \\
& Robot (Mosaic) & 94.60 & 98.00 & 90.00 & 100.00 & 80.00 & 100.00 & 98.00 & 88.00 & 100.00 & 100.00 & 92.00 \\
\cmidrule{2-13}
& Robot w/o Gripper (BG) & 90.60 & 90.00 & 96.00 & 94.00 & 72.00 & 98.00 & 92.00 & 78.00 & 96.00 & 100.00 & 90.00 \\
& Robot w/o Gripper (Black) & 92.60 & 100.00 & 94.00 & 96.00 & 78.00 & 96.00 & 94.00 & 78.00 & 100.00 & 96.00 & 94.00 \\
& Robot w/o Gripper (Mosaic) & 96.40 & 92.00 & 100.00 & 100.00 & 92.00 & 98.00 & 98.00 & 90.00 & 100.00 & 100.00 & 94.00 \\
\cmidrule{2-13}
& Background (Black) & 72.20 & 86.00 & 98.00 & 34.00 & 52.00 & 96.00 & 96.00 & 56.00 & 22.00 & 100.00 & 82.00 \\
& Background (Mosaic) & 97.60 & 98.00 & 100.00 & 96.00 & 94.00 & 100.00 & 100.00 & 90.00 & 98.00 & 100.00 & 100.00 \\

\bottomrule
\end{tabular}
\caption{Success rates (\%) across tasks and masking strategies on \textbf{LIBERO-Goal} for OpenVLA-OFT. The instruction is provided in Table \ref{tab:patch_mask_goal_ins}.} \label{tab:mask_goal_oft}
\end{table*}


==> tabs/pi05_attention_stage.tex <==
\begin{table*}[t]
\centering
\small
\begin{tabular}{llccc}
\toprule
Model / analysis & Region or quantity & Phase 1 & Phase 2 & Full rollout \\
\midrule
\multirow{5}{*}{$\pifive$ attention mass}
& GT union & 0.6566 & 0.6373 & 0.6469 \\
& Gripper & 0.2128 & 0.1594 & 0.1860 \\
& Robot arm & 0.1756 & 0.1983 & 0.1870 \\
& Manipulated object & 0.1343 & 0.1316 & 0.1329 \\
& Receptacle / affordance & 0.1339 & 0.1480 & 0.1409 \\
\midrule
\multirow{4}{*}{$\pifive$ stage tracking}
& Successful rollouts / analyzed steps & \multicolumn{3}{c}{10 / 2632} \\
& Mean GT-union mass across tasks & \multicolumn{3}{c}{0.6469 $\pm$ 0.0187} \\
& Mean subtask focus-set mass & \multicolumn{3}{c}{0.2224} \\
& Active-object advantage over next-stage object & \multicolumn{3}{c}{0.0610 (max 0.1067)} \\
\midrule
OpenVLA rollout evidence & Pretrained / fine-tuned success & \multicolumn{3}{c}{0 / 50 \quad vs. \quad 31 / 50} \\
\bottomrule
\end{tabular}
\caption{Attention-mass and rollout-stage statistics from the supporting analyses. Unlike Top-10 patch IoU, attention mass preserves the continuous action-to-image heatmap and reports the fraction of total attention assigned to each simulator-derived region.}
\label{tab:attention_stage}
\end{table*}

==> tabs/robotwin_instruction.tex <==
% \begin{table*}[t]
% % \begin{table}[t]
% \centering
% \footnotesize
% \setlength{\tabcolsep}{4pt}
% \renewcommand{\arraystretch}{1.12}

% \begin{tabularx}{\textwidth}{p{1.0cm} Y p{3.0cm}}
% \toprule
% \textbf{ID} & \textbf{Instruction} & \textbf{Capability} \\
% \midrule
% t0 & Click the alarm clock's center of the top side button on the table. & Button clicking \\
% t1 & Click the bell's top center on the table. & Target clicking \\
% t2 & Use both arms to grab the roller on the table. & Bimanual grasping \\
% t3 & Use both arms to lift the pot. & Bimanual lifting \\
% t4 & Use one arm to press the stapler. & Single-arm pressing \\
% \bottomrule
% \end{tabularx}

% \caption{Overview of the selected RoboTwin2.0 manipulation tasks.}
% \label{tab:robotwin_tasks}
% \end{table*}
\begin{table*}[t]
\centering
\footnotesize
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.12}

\begin{tabularx}{\textwidth}
{p{2.0cm} p{0.7cm} X p{2.8cm}}
\toprule
\textbf{Benchmark} &
\textbf{ID} &
\textbf{Instruction} &
\textbf{Capability} \\
\midrule

\multirow{5}{*}{\makecell[l]{\textbf{RoboTwin2.0}\\Dual-arm}}
&t0 & Click the alarm clock's center of the top side button on the table. &
Button clicking \\

&t1 & Click the bell's top center on the table. &
Target clicking \\

&t2 & Use both arms to grab the roller on the table. &
Bimanual grasping \\

&t3 & Use both arms to lift the pot. &
Bimanual lifting \\

&t4 & Use one arm to press the stapler. &
Single-arm pressing \\

\midrule

\multirow{4}{*}{\makecell[l]{\textbf{Simpler}\\Real-to-Sim}}
&t0 & Put carrot on plate. &
Object placement \\

&t1 & Put eggplant into yellow basket. &
Goal-conditioned manipulation \\

&t2 & Put the spoon on the towel. &
Spatial reasoning \\

&t3 & Stack the green block on the yellow block. &
Stacking / compositional manipulation \\

\bottomrule
\end{tabularx}

\caption{
Overview of evaluated embodied manipulation tasks.
RoboTwin2.0 primarily evaluates real-world dexterous manipulation,
with particular emphasis on dual-arm environment and fine-grained interaction skills.
In contrast, SimplerEnv is designed as a scalable real-to-simulation benchmark,
focusing on policy generalization and robustness under distribution shifts,
where simulated performance is expected to correlate with real-world execution.
}
\label{tab:robotwin_simpler}
\end{table*}

==> tabs/summary_2.tex <==
\begin{table*}[t]
\centering
\small
\renewcommand{\arraystretch}{1.25}
\setlength{\tabcolsep}{5pt}

\begin{tabular}{p{2.8cm} p{3.2cm} p{3.5cm} p{2.5cm} p{2.8cm}}
\toprule
\textbf{Research Question} &
\textbf{Analysis Probe} &
\textbf{Key Evidence / Finding} &
\textbf{Benchmark} &
\textbf{Model Coverage} \\
\midrule

\multirow{2}{*}{
\makecell[l]{\textbf{RQ1}\\Representation\\Geometry}
}
& Cross-Modal CKA
& Cross-modal alignment patterns
& LIBERO, COCO
& $\pi_{0.5}$, OpenVLA \\

& Checkpoint-Drift CKA
& Representation evolution during adaptation
&
& \\

\midrule

\multirow{2}{*}{
\makecell[l]{\textbf{RQ2}\\Causal Control\\Attribution}
}
& Attention Knockout
& Modality dependence of action generation
& LIBERO, CALVIN,
RoboTwin2.0
& $\pi_{0.5}$, OpenVLA, OFT \\

& Layer-wise Knockout
& Hierarchical control attribution
&
& \\

\midrule

\multirow{3}{*}{
\makecell[l]{\textbf{RQ3}\\Behavioral\\Manifestation}
}
& Attention IoU + Visualization
& Spatial-temporal attention consistency
& LIBERO-10
& \multirow{3}{*}{
\makecell[c]{
$\pi_{0.5}$\\
OpenVLA\\
OFT\\
X-VLA
}
}
\\

& Visual Patch Mask
& Shortcut dependence and visual robustness
& LIBERO, CALVIN,
Simpler, RoboTwin2.0
& \\

& Input Editing
& Instruction sensitivity and semantic grounding
& LIBERO-10
& \\

\bottomrule
\end{tabular}

\caption{
Overview of the VLA-Trace framework organized as a progressive mechanistic evidence chain:
(1) representation geometry analysis,
(2) causal attribution of action generation,
and (3) behavioral manifestation of shortcut dependence.
The framework progressively links internal representations,
control mechanisms, and observable behaviors across multiple embodied benchmarks.
}
\label{tab:vlatrace}
\end{table*}
